Offensive Robot Cybersecurity

Offensive Robot Cybersecurity introduces a groundbreaking approach by advocating for offensive security methods empowered by means of automation. It emphasizes the necessity of understanding attackers' tactics and identifying vulnerabilities in advance to develop effective defenses, thereby improving robots' security posture. This thesis leverages a decade of robotics experience, employing Machine Learning and Game Theory to streamline the vulnerability identification and exploitation process. Intrinsically, the thesis uncovers a profound connection between robotic architecture and cybersecurity, highlighting that the design and creation aspect of robotics deeply intertwines with its protection against attacks. This duality -- whereby the architecture that shapes robot behavior and capabilities also necessitates a defense mechanism through offensive and defensive cybersecurity strategies -- creates a unique equilibrium. Approaching cybersecurity with a dual perspective of defense and attack, rooted in an understanding of systems architecture, has been pivotal. Through comprehensive analysis, including ethical considerations, the development of security tools, and executing cyber attacks on robot software, hardware, and industry deployments, this thesis proposes a novel architecture for cybersecurity cognitive engines. These engines, powered by advanced game theory and machine learning, pave the way for autonomous offensive cybersecurity strategies for robots, marking a significant shift towards self-defending robotic systems. This research not only underscores the importance of offensive measures in enhancing robot cybersecurity but also sets the stage for future advancements where robots are not just resilient to cyber threats but are equipped to autonomously safeguard themselves.

==> figures/ris.tex <==
\begin{figure}[h!]
    \centering % Centers the figure
   
    \begin{tikzpicture}[node distance=2cm, auto, scale=0.5, transform shape]
        % Styles for nodes and lines
        \tikzstyle{box} = [rectangle, draw, fill=gray!20, text centered, rounded corners, minimum height=2.5em, minimum width=3cm]
        \tikzstyle{emphasize} = [box, fill=blue!30, draw=blue, line width=1.5pt]
        \tikzstyle{line} = [draw, -{Latex[scale=1.2]}]
        \tikzstyle{deemphasize} = [opacity=0.3]
        \tikzstyle{innerComp} = [rectangle, draw, fill=orange!30, text centered, minimum height=1.5em, minimum width=3em]
        \tikzstyle{innerComp_emphasize} = [rectangle, fill=blue!30, draw=blue, line width=1.5pt]
    
        % Nodes
        \node[box] (U) {User};
        \node[box, emphasize] (EF) at (11cm,0) {1. ExploitFlow}; 
        \node[box, emphasize, below left=4cm and 2.5cm of EF] (PentestGPT) {2. PentestGPT};
        \node[box, emphasize, below=8cm of EF] (PentestPerf) {3. PentestPerf};
        \node[box, right=3cm of EF] (T) {Target};
    
        % Inner components of EF
        \node[innerComp, above=2.5cm of EF, xshift=-4cm] (exploit) {exploit};
        \node[innerComp, right of=exploit] (flow) {flow};
        \node[innerComp, right of=flow] (graph) {graph};
        \node[innerComp, right of=graph] (adapters) {adapters};
        \node[innerComp, right of=adapters] (models) {models};
        \node[innerComp, right of=models] (state) {state};
        \node[innerComp, below=0.5cm of EF, xshift=3.5cm] (gt) {Game Theory (\CutTheRope)};
    
        % Inner components of PentestGPT
        \node[innerComp, above=2.5cm of PentestGPT, xshift=-2cm] (parsing) {parsing};
        \node[innerComp, right of=parsing] (reasoning) {reasoning};
        \node[innerComp, right of=reasoning] (generation) {generation};
    
        % Dashed lines connecting to inner components
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (exploit);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (flow);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (graph);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (adapters);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (models);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (state);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (gt);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (PentestGPT) -- (gt);        
    
        \draw[dashed, shorten <=5pt, shorten >=5pt] (PentestGPT) -- (parsing);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (PentestGPT) -- (reasoning);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (PentestGPT) -- (generation);

        % Group/box around EF and PentestGPT
        \node[rectangle, fill=gray!5, draw, dashed, deemphasize, fit=(EF) (PentestGPT), inner sep=1cm] (group) {};
        \node[anchor=north west, inner sep=0.5cm] at (group.south west) {4. Malism};
    
        % Lines
        \path[line] (U) -- node[font=\small, midway, sloped, above] {programatically in Python} (EF); 
        \path[line] (U) edge[bend right=40] node[font=\small, sloped, below] {goal description in text} (PentestGPT);
        \path[line] (PentestGPT) edge[bend right=20] node[font=\small, sloped, below] {exchange exploit tree} (EF);
        \path[line] (EF) edge[bend left=20] node {} (PentestGPT);
        \path[line] (EF) -- node[font=\small, sloped, above] {Benchmarks an exploit flow} (PentestPerf);
        \path[line] (EF) -- (T);
        \path[line] (T) -- (EF);
    
    
        % re-draw
        \node[box, emphasize, below left=4cm and 2.5cm of EF] (PentestGPT) {2. PentestGPT};
        \node[innerComp, below=0.5cm of EF, xshift=3.5cm] (gt) {Game Theory (\CutTheRope)};
        \node[box, emphasize] (EF) at (11cm,0) {1. ExploitFlow}; 

        \node[innerComp, above=2.5cm of PentestGPT, xshift=-2cm] (parsing) {parsing};
        \node[innerComp, right of=parsing] (reasoning) {reasoning};
        \node[innerComp, right of=reasoning] (generation) {generation};
        
        % Legend
        \begin{scope}[node distance=0.3cm, font=\footnotesize]
            \coordinate (legendOrigin) at (-4,-6); % Set the position for the start of the legend
            \node[box, right=0.3cm of legendOrigin, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendBox) {}; 
            \node[right=0.3cm of legendBox] {External entity};
    
            %\node[box, below=0.2cm of legendBox, fill=gray!5, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (otherpapers) {}; 
            %\node[right=0.3cm of otherpapers] {Other future papers};
    
            \node[emphasize, below=0.2cm of legendBox, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendEmphasize) {};
            \node[right=0.3cm of legendEmphasize] {Developed in this thesis};
    
            \node[innerComp, below=0.2cm of legendEmphasize, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendInner) {};
            \node[right=0.3cm of legendInner] {Inner Component};

            % Final comments clarifying in which chapter it's developed            
            %\node[right=0.5cm of PentestPerf, text width=2cm, opacity=0.7] {Developed in chapter X, alongside PentestGPT};            
            
        \end{scope}
    \end{tikzpicture}
    
    \caption{
        Our architecture and framework to develop fully automated offensive robot cybersecurity agents, which name \emph{cybersecurity cognitive engines} in Chapter \ref{chapter:game_theory}: \framework{}.
    }
    \label{figure:cybersecurity_cognitive_engine:conclusion} % Label to reference the figure elsewhere
    % \label{figure:cybersecurity_cognitive_engine:machine_learning}
\end{figure}

==> sections/I.motivation/rosdiagram.tex <==
\begin{figure}[!h]
    \centering
    \scalebox{0.45}{
    \tikzset{
      state/.style={
        rectangle, rounded corners, draw=gray!80, gray!20, thick,
        minimum height=2em, inner sep=10pt, text centered},
      state2/.style={
        rectangle, rounded corners, draw=black, fill=gray!70, thick,
        minimum height=2em, inner sep=10pt, text centered},
      epath/.style={draw, <->, shorten <=1pt, shorten >=1pt},
      cir/.style={draw, circle, fill, inner sep=2.5pt, text=white},
      fpath/.style={draw, color=gray, rounded corners=3pt, shorten <=3pt, shorten >=3pt, align = center, minimum height = 10pt, font = \bfseries},
      dir/.style={near start, right, font=\small},
    }
    \begin{tikzpicture}[->, >=latex, line width=0.75pt]
      \draw[fill=white, color=white] (-10.8,-4.5) rectangle (9.2,4.5);
      
      %%%%%%%%%
      % titles
      %%%%%%%%%      
      %\node[text width=2.5cm] (mug) at (12.6,-4.7) {\Huge ROS 2\\ HAWG};
      %\node[text width=3.5cm] (mug) at (-12.6,9.7) {\Large ROS 2 stack};
      %\node[text width=3.5cm] (mug) at (-12..,14.7) {\Huge \tt OSI\\stack};
      %\node[text width=3.5cm] (mug) at (-12.,14.7) {\Huge \tt ROS 2\\stack};
      %\node[text width=3.5cm] (mug) at (1.,14.7) {\Huge \tt KRS\\stack};
      
      %\node[text width=2.5cm] (pilar1) at (-5.6,-4.7) {\Large pilar I};
      %\node[text width=2.5cm] (pilar2) at (1.0,-4.7) {\Large pilar II};
      %\node[text width=2.5cm] (pilar3) at (9.0,-4.7) {\Large pilar III};
      
      %\node[rotate=90] (site) at (-10.6, 5) {
      %  \large github.com/ros-acceleration %\hspace{3ex} www.xilinx.com
      %};
      

    %%%%%%%%%%%
    % build system
    %%%%%%%%%%%
    % build system
    \node[state, text width=7cm, text ragged, fill=black!40]
        (buildsystem) at (-6.4, 2.) {
            {build system (\texttt{ament})}\\
    };
    % ament_acceleration
    \node[state, text width=7cm, fill=black!40]
        (amentacceleration) at (-6.4, 3.2) {
            {\tt ament\_acceleration}\\
    };

    % ament_vitis
    \node[state, text width=2.2cm, text height=1cm, fill=black!40]
        (amentvitis) at (-8.8, 4.7) {
            {\tt ament\_vitis}\\
    };

    % ament_rocm
    \node[state, text width=2cm, text height=1cm, fill=black!40]
        (amentrocm) at (-5.8, 4.7) {
            {\tt ament\_rocm}\\
    };

    % ament_more
    \node[state, text width=1.cm, text height=1cm, fill=black!40]
        (amentmore) at (-3.4, 4.7) {
            {\tt ...}\\
    };
    
    %%%%%%%%%%%
    % colcon - metabuild
    %%%%%%%%%%%
    \node[state, text width=4.3cm, text ragged, fill=black!40]
        (metabuild) at (0.2, 2.) {
        {meta build (\texttt{colcon})}\\
    };

    % colcon_acceleration
    \node[state, text width=4.3cm, text ragged, fill=black!40]
        (colconaccel) at (0.2, 3.2) {
        {\tt colcon\_acceleration}\\
    };
    
    % vitis
    \node[state, text width=4.3cm, text ragged, fill=black!40] (vitis) at (0.2, 4.7) {
        \texttt{Vitis \\Unified Software\\ Platform}
    };


    %%%%%%%%%%%
    % firmware
    %%%%%%%%%%%
    \node[state, text width=10cm, text ragged, fill=black!40]
    (firmware) at (8.3, 2.) {
        {firmware}\\
    };
    \node[state, text width=10cm, fill=black!40]
    (accelerationfirmware) at (8.3, 3.2) {
        {\tt acceleration\_firmware}\\
    };
    \node[state, text width=3.5cm, text height=0.5cm, fill=black!40]
        (accelerationfirmwarekv260) at (5.0, 4.7) {
            {\tt acceleration\_\\firmware\_kv260}
    };
    \node[state, text width=3.5cm, text height=0.5cm, fill=black!40]
        (accelerationfirmwarezcu102) at (9.4, 4.7) {
            {\tt acceleration\_\\firmware\_zcu102}
    };
    \node[state, text width=1.2cm, text height=1cm, fill=black!40]
        (accelerationfirmwaremore) at (12.7, 4.7) {
            {\tt ...}
    };

    %%%%%%%%%%%
    % userland
    %%%%%%%%%%%
    % drivers
    \node[state, text width=7cm, text ragged, fill=black!40]
        (driver) at (-6.4, 6.3) {
            {drivers}\\
    };
    \node[state, text width=4.3cm, text ragged, fill=black!40]
        (libraries) at (0.2, 6.3) {
        {libraries}\\
    };
    \node[state, text width=10cm, text ragged, fill=black!40]
    (cloud) at (8.3, 6.3) {
        {cloud}\\
    };
    \node[state, text width=12cm, text ragged, fill=black!40]
        (accelerationexamples) at (-3.9, 7.5) {
            {\tt acceleration\_examples}\\
    };


    %%%%%%%%%%%
    % KRS components
    %%%%%%%%%%%

    %% rcl
    \node[state, text width=23.3cm, text height=0.2cm, fill=black!40]
      (rclkrs) at (1.7, 0.8) {
        {\tt ROS Client Library (rcl)}\\
    };
    
    %% rmw
    \node[state, text width=23.3cm, text height=0.2cm, fill=black!40]
      (rmwkrs) at (1.7, -0.3) {
        {\tt ROS MiddleWare interface (rmw)}\\
    };
    
    % DDS impl. 1 adapter
    \node[state, text width=7cm, text, text height=0.2cm, fill=black!40]
        (dds1adapter) at (-6.45, -1.39) {
            {DDS impl. 1 adapter (\texttt{rmw\_<dds1>})}\\
    };
    % DDS impl. 1
    \node[state, text width=7cm, text height=1cm, fill=black!40]
      (dds1) at (-6.45,-2.8) {
        {\tt DDS implementation 1}\\
    };

    % DDS impl. ... adapter
    \node[state, text width=0.3cm, text, text height=0.2cm, fill=black!40]
        (ddsoadapter) at (-1.9, -1.39) {
            {...}\\
    };
    % DDS impl. ...
    \node[state, text width=0.3cm, text height=1cm, fill=black!40]
      (ddso) at (-1.9,-2.8) {
        {...}\\
    };

    % DDS impl. n adapter
    \node[state, text width=3.5cm, text, text height=0.2cm, fill=black!40]
        (ddnsadapter) at (0.9, -1.39) {
            {DDS impl. \texttt{n} adapter}\\
    };
    % DDS impl. n
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (ddns) at (0.9,-2.8) {
        {\tt DDS implementation n}\\
    };

    % iceoryx adapter
    \node[state, text width=3.5cm, text, text height=0.2cm, text width=7cm, fill=black!40]
        (iceoryxadapter) at (7.0, -1.39) {
            {Eclipse iceoryx™ adapter (\texttt{rmw\_iceoryx})}\\
    };
    % iceoryx
    \node[state, text width=3.5cm, text height=1cm, text width=7cm, fill=black!40]
      (iceoryx) at (7.0,-2.8) {
        {\tt Eclipse iceoryx™}\\
    };
    
    % XRT
    \node[state, text width=3.5cm, text, text height=1.1cm, text width=2.0cm, fill=black!40]
        (xrt) at (12.4, -2.3) {
            {Xilix Runtime \\(\texttt{XRT})}\\
    };

    % Yocto/PetaLinux
    \node[state, text width=11.6cm, text height=1.0cm, text, fill=black!40]
        (petalinux) at (-4.1, -4.7) {
            {Yocto/PetaLinux    }\\
    };

    % Ubuntu Linux
    \node[state, text width=10.9cm, text height=1.0cm, text, fill=black!40]
        (ubuntu) at (8.0, -4.7) {
            {Ubuntu Linux}\\
    };
    
    % LNS
    \node[state, text width=23.3cm, text height=1.0cm, fill=black!40]
      (lns) at (1.7, -6.6) {
            {Linux Networking Stack (LNS)}\\
    };
    
    %% Link layer
    % Ethernet
    \node[state, text width=3.5cm, text height=1.0cm, fill=black!40]
      (ethernet) at (-8.2, -8.5) {
            {Ethernet}\\
    };
    % TSN
    \node[state, text width=3.5cm, text height=0.55cm, fill=black!40]
      (tsn) at (-3.8, -8.5) {
            {Time Sensitive Networking (TSN)}\\
    };
    % EtherCAT
    \node[state, text width=3.5cm, text height=1.0cm, fill=black!40]
      (ethercat) at (0.6, -8.5) {
            {EtherCAT}\\
    };
    % CAN
    \node[state, text width=3.5cm, text height=1.0cm, fill=black!40]
      (can) at (5.0, -8.5) {
            {CAN}\\
    };
    % ...
    \node[state, text width=5.7cm, text height=1.0cm, fill=black!40]
      (otherlink) at (10.5, -8.5) {
            {...}\\
    };
    
    % xen
    \node[state, text width=23.3cm, text height=0.2cm, fill=black!40]
      (xen) at (1.7, -10.0) {
        {\tt Xen hypervisor}\\
    };


    %% Hardware
    % KV260
    \node[state, text width=11.6cm, text height=1.0cm, fill=black!40]
      (kv260) at (-4.1, -11.5) {
            {KV260}\\
    };
    % 
    \node[state, text width=10.8cm, text height=1.0cm, fill=black!40]
      (k26) at (7.9, -11.5) {
            {K26 SOM}\\
    };
    
    % ZCU102
    %\node[state, text width=3.5cm, text height=1.0cm, fill=Gray!30]
    %  (zcu102) at (0.6, -11.5) {
    %        {ZCU102}\\
    %};
    % ZCU104
    %\node[state, text width=3.5cm, text height=1.0cm, fill=Gray!30]
    %  (zcu104) at (5.0, -11.5) {
    %        {ZCU104}\\
    %};
    % ...
    %\node[state, text width=5.7cm, text height=1.0cm, fill=Gray!30]
    %  (otherhw) at (10.5, -11.5) {
    %        {...}\\
    %};

    
    %%%%%%%%%%%
    % OSI stack
    %%%%%%%%%%%
    %% 7. Application
    \node[state, text width=3.2cm, text height=14.5cm, fill=black!60]
      (osil7) at (-12.9, 5.6) {
        {\tt 7. Application}\\
    };
    
    %% 6. Presentation
    \node[state, text width=3.2cm, fill=black!60]
      (osil6) at (-12.9, -2.7) {
        {\tt 6. Presentation}\\
    };

    %% 5. Session
    \node[state, text width=3.2cm, fill=black!60]
      (osil5) at (-12.9, -3.8) {
        {\tt 5. Session}\\
    };

    %% 4. Transport
    \node[state, text width=3.2cm, text height=1cm, fill=black!60]
      (osil4) at (-12.9, -5.3) {
        {\tt 4. Transport}\\
    };

    %% 3. Network
    \node[state, text width=3.2cm, fill=black!60]
      (osil3) at (-12.9, -6.8) {
        {\tt 3. Network}\\
    };

    %% 2. Data Link
    \node[state, text width=3.2cm, fill=black!60]
      (osil2) at (-12.9, -7.9) {
        {\tt 2. Data Link}\\
    };

    %% 1. Physical
    \node[state, text width=3.2cm, text height=3cm, fill=black!60]
      (osil1) at (-12.9, -10.5) {
        {\tt 1. Physical}\\
    };

    %%%%%%%%%%%
    % App Store
    %%%%%%%%%%%
    %% Xilinx App Store
    \node[state, text width=18.9cm, text height=0.2cm, fill=black!40]
      (embeddedappstore) at (-0.5, 8.7) {
        {\tt Xilinx App Store}\\
    };
    
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (navstackaccel) at (-8.2, 10.3) {
            {Accelerator \#1 for \texttt{navigation stack}}\\
    };
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (navstackaccel2) at (-8.2, 12.3) {
            {Accelerator \#2 for \texttt{navigation stack}}\\
    };

    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (manaccel) at (-3.8, 10.3) {
            {Accelerator \#1 for \texttt{manipulation stack}}\\
    };

    %\node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
    %  (controlaccel) at (0.6, 10.3) {
    %        {Accelerator \#1 for \texttt{control stack}}\\
    %};

    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (perceptaccel) at (0.6, 10.3) {
            {Accelerator \#1 for \texttt{perception stack}}\\
    };
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (perceptaccel2) at (0.6, 12.3) {
            {Accelerator \#2 for \texttt{perception stack}}\\
    };

    \node[state, text width=5.7cm, text height=0.6cm, fill=black!40]
      (actaccel) at (6.1, 10.3) { % 10.5
            {Accelerator \#1 for \\ \texttt{actuator} \#1}\\
    };    
    \node[state, text width=5.7cm, text height=0.6cm, fill=black!40]
      (actaccel2) at (6.1, 12.3) {
            {Accelerator \#2 for \\ \texttt{actuator} \#1}\\
    };

    % non-app store    
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (accapp1) at (11.6, 9.1) {
            {Robot accelerated \\ application \#n}\\
    };    
    \node[state, text width=3.5cm, text height=0.6cm, fill=black!40]
      (accapp1) at (11.6, 11.1) {
            {Accelerator \#n for \\ application \#n}\\
    };    
    

    %%%%%%%%%%%%
    % paths
    %%%%%%%%%%%%


    %\path[fpath, color=Maroon, text width = 8cm] (a) -- ($(a)+(5.85,0)$) node[dir, right, at end] {\texttt{ament\_vitis} macro, helps define accelerators directly from CMakeList.txt};
    
    % applications/libraries indeterminism
    \path[-, dashed, fpath, color=black] (actaccel2) -- ($(actaccel2)+(8.5,0)$) |-
            node[dir, text width=4cm] {\Large \circledgray{7} \textbf{OSI L7} robotics application/libraries indeterminism} (cloud);

    % ROS 2 indeterminism
    \path[-, dashed, fpath, color=black] (firmware) -- ($(firmware)+(6.25,0)$) |-
            node[dir, text width=4cm] {\Large \circledgray{6} \textbf{OSI L7} \\ ROS 2 core layers indeterminism} (iceoryxadapter);


    % Comm. middleware indeterminism
    \path[-, dashed, fpath, color=black] ($(iceoryx)+(3,1)$) -- ($(iceoryx)+(7.5,1)$) |-
            node[dir, text width=4cm] {\Large \circledgray{5} \textbf{OSI L5-L7} \\ communication middleware indeterminism} ($(ubuntu)+(2,1)$);


    % Last-level cache contention
    \path[-, dashed, fpath, color=black] ($(navstackaccel2)+(-0,0.5)$) -- ($(navstackaccel2)+(-11.0,0.7)$) |-
            node[dir, text width=4cm] {\Large \circledgray{4} \textbf{OSI L3-L7} \\ last-level cache contention} ($(xen)+(2,-0.5)$);

    % Linux kernel indeterminism
    \path[-, dashed, fpath, color=black] ($(ubuntu)+(3,0.7)$) -- ($(ubuntu)+(6.5,0.7)$) |-
            node[dir, text width=4cm] {\Large \circledgray{3} \textbf{OSI L3-L7} \\ Linux kernel indeterminism} ($(lns)+(2,1)$);

    % LNS
    \path[-, dashed, fpath, color=black] ($(lns)+(5,1.0)$) -- ($(lns)+(12.7,1.0)$) |-
            node[dir, text width=5cm] {\Large \circledgray{2} \textbf{OSI L3-L4} \\ Linux Networking Stack (LNS) queues} ($(otherlink)+(2,1)$);

    % Link layer congestion bottlenecks
    \path[-, dashed, fpath, color=black] ($(otherlink)+(1,1.0)$) -- ($(otherlink)+(3.9,1.0)$) |-
            node[dir, text width=5cm] {\Large \circledgray{1} \textbf{OSI L2} \\ Link layer congestion bottlenecks} ($(otherlink)+(2,-1)$);


    %%%%%%%%%%%%
    % arrows  
    %%%%%%%%%%%%
    %\draw[<-, rounded corners] (-7.15,-1.2) |- ++(-0.5,-0.7) -| (amentvitis);
    

    %\path[black, epath] (vitis) to[out=-60, in=120] node[cir, pos=0.4] {3} (amentmore);
    
    %\path[black, epath] (vitis) to[out=150, in=90](amentvitis);


    % pillars
    %\path[gray, dashed, epath] (pilar1) to[out=120, in=270](buildsystem);
    %\path[gray, dashed, epath] (pilar2) to[out=120, in=270](metabuild);
    %\path[gray, dashed, epath] (pilar3) to[out=120, in=270](firmware);


    \end{tikzpicture}}
    \caption{The ROS 2 robotics stack.}
    \label{fig:ros2}
\end{figure}

==> sections/II.ethics/X.obsolescence.tex <==
\chapter{Planned obsolescence}
\label{chapter:obsolescence}

%As robots get damaged or security compromised, their components will increasingly require updates and replacements. Contrary to the expectations, most manufacturers employ planned obsolescence practices and discourage repairs to evade competition. We introduce and advocate for \emph{robot teardown} as an approach to study robot hardware architectures and fuel security research. We show how our approach helps uncovering security vulnerabilities, and provide evidence of planned obsolescence practices.

\section{Introduction}
%\label{sec:introduction}

A robot is a network of networks, with sensors, actuators, and dedicated computing resources, according to its application. A robotic manipulator, for instance, include the arm's mechanics (which generally include actuators and sensors), the Human-Machine Interface (HMI), the controller (the main compute substrate for reasoning), and any additional safety mechanism. Most industrial robots of this kind range from tenths to hundreds of thousands of Euros. Accordingly, it is only reasonable to consider the need for repairing robots.

%As part of the Circular Economy Action Plan~\cite{eccircularap}, the EC has shown commitment towards establishing a new '\emph{Right to Repair}' in the context of reviewing directive 2019/771~\cite{cordella2019analysis}.
%In the US, it wasn't until 2012 that the Automotive \emph{Right to Repair} passed in Massachussets~\cite{hatta2020right}, empowering customers with tools to fight planned obsolescence.

Unfortunately, relevant robot manufacturers follow planned obsolescence practices nowadays and organize approved distributors and integrators into private networks, providing repair parts only to \emph{certified} companies.
Among the most recent examples we observe the case of Teradyne, which robots are advertised as collaborative (i.e., designed to safely work in close contact with humans), while research unveils that they lack of safety measures~\cite{mayoral2019industrial} and a concerning cybersecurity~\cite{kirschgens2018robot} landscape.

Given these premises, we promote robot teardown as a systematic \emph{process} to repair robots, improve robot hardware and research its security.
In the long run, we argue that the more researchers and practitioners will get used to systematically teardown robots, the more this practice will impact the quality assurance of hardware in robotics, putting pressure on manufacturers to produce robots with better hardware security measures, thereby safer.

\section{Robot teardown\vspace{-0.5em}}
A \textit{robot teardown} is the process of analyzing a robot's hardware architecture to model its functional behavior and physical components, through systematic disassembling.
We identify three key purposes in robotics: a) dissection and analysis to evaluate the status of a product, b) competitive benchmarking against similar products, and c) gain engineering experience and knowledge.
We focus on a) and c) through three case studies on the robots from Universal Robots (UR) and Mobile Industrial Robots (MiR), which have tenths of thousands of units sold and operating in close contact with humans (as collaborative robots), and have been already shown lacking security measures \cite{vilches2019introducing} from these two manufacturers. 

Due to space limitations, we leave the complete walk-through of these case studies to an extended version of this paper, focusing now only on the outcome.


\begin{figure*}[!h]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ur1.png}
        \label{fig:tear:1}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ur5.png}
        %\caption{\footnotesize \textbf{UR3 CB series}: The safety side of the controller (documented in the user manuals) includes quick connectors which can be removed by carefully wiggling them out.}
        \label{fig:tear:2}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ur9.png}
        %\caption{\footnotesize \textbf{UR3 CB series}: Final figure depicting all the components contained inside of the Universal Robots UR3 CB3.1 controller, except for the teach pendant.}
        \label{fig:tear:3}
    \end{subfigure}
    %\\[3ex]
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ure2.png}
        %\caption{\footnotesize \textbf{UR3e e-Series}: Inside the controller we can see various connectors and cables exposed. The right side includes I/O and safety, at the bottom USB, HMI and SD card.}
        \label{fig:tear:4}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ure11.png}
        %\caption{\footnotesize \textbf{UR3e e-Series}: Even though from a first look, the pin-out seems similar to previous iterations of the CB3 controller, the connector itself has a different shape.}
        \label{fig:tear:5}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/ur3e_motor.jpg}
        %\caption{\footnotesize \textbf{UR3e e-Series}: Opening a joint we find the harmonic drive, on top of the \ac{PCB} for communication and power distribution. And the release solenoid.}
        \label{fig:tear:6}
    \end{subfigure}
    %\\[3ex]
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/mir1.png}
        \label{fig:tear:7}
        %\caption{\footnotesize \textbf{MiR-100}: The top shell sits on top of a metal frame that protects all the electronic components. Simply lifting the top shell reveals the internal electronic components.}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/mir2.png}
        %\caption{\footnotesize \textbf{MiR-100}: A circuit-breaker switch is present to disconnect the main power line going from the batteries to the rest of the robot. A quick-release connector is also present.}
        \label{fig:tear:8}
    \end{subfigure}    
    ~
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/mir8.png}
        %\caption{\footnotesize \textbf{MiR100}: Final disassembly  depicting  some of the main components contained inside of  the  MiR100 industrial mobile robot, alongside the tools used for the teardown.}
        \label{fig:tear:9}
    \end{subfigure}    
    
    
    \caption{Obsolescense evidence from three industrial collaborative robots: UR3 CB series (first three), UR3e e-Series (fourth to sixth) and MiR100 (last three).}
    \label{figure:obsolescense}
\end{figure*}

\vspace{-1.5em}

\subsection{Case Study 1: Teardown of an industrial collaborative robot}

The safety logic of the UR3 CB-Series collaborative robot runs on a NXP LPC4437JET256 microcontroller, which datasheet\footnote{\url{https://www.nxp.com/docs/en/data-sheet/LPC435X_3X_2X_1X.pdf}} highlights that the microcontroller is not suitable for safety-critical systems according to the silicon vendor. This leads us to question the quality and reliability of the safety implementation within these robots. Therefore, through teardown, we were able to identify and pinpoint hardware components that don't meet the quality standards for the safety situations the robot may have to face, leading to an overall improved scenario for end-users.

\subsection{Case Study 2: Teardown of a next-gen industrial collaborative robot}
Following the CB-Series, we proceeded and disassembled one of the latest releases from Universal Robots, the UR3e, an e-Series. While the external look remains similar, the internals have changed significantly: 1) The e-Series controller integrates a single PSU, while the CB-series had two, 2) while the CB-Series presented two boards containing compute, power, and safety logic, the e-Series presents only one single PCB featuring a Xilinx Artix-7 series FPGA, widely used for implementing safety logic in a variety of automotive and control domains, 3) the base filter PCB---which helps interface power and RS485 communications from the controller (e-Series) to the robot arm mechanics---is similar to the one present in the CB-series, 4) the arm's mechanics connector changed in the e-Series but the power and communications lines remain coherent (through the base filter board) and 5) the electronics within the arm's mechanics do not present relevant changes from an interoperability perspective, which should facilitate re-purposing and reuse.

\subsection{Case Study 3: Teardown of a mobile industrial robot}
\label{mirdissasembly}

The MiR-100 is a popular mobile robot manufactured by the Danish Mobile Industrial Robots (MiR), also owned by the US Teradyne.
The first impression is that various components of the robot could be improved from a safety perspective. Also, the teardown helped understand how this robot presents multiple (internal and external) networks and how each one of the sensors and actuators are connected across these networks, forming the data layer graph. The robot itself is powered by ROS~\cite{Quigley09} and gaining further understanding of the ROS computational graph requires understanding also its underlying hardware mapping (from which one derives the data layer graph).
The teardown exercise supplies exactly this and allows to produce a data layer graph represented in the form of a hardware schematic which can then be used in combination with the computational graph to gain further understanding of the robot.

\vspace{-0.5em}

\section{Teardown to research security and identify planned obsolescence}
\label{sec:obsolescence}

\vspace{-0.5em}

Teardown supports Kerckhoffs' principle in revealing all the details and weaknesses of a security system, excluding volatile secrets such as keys or credentials stored in memory.
Overall, the history of proprietary systems violating Kerckhoffs' principle by pursuing security-by-obscurity is rich of failure cases (with the military domain as the sole exception). As part of this research, our group identified more than 100 security flaws across the three robots described above over a period of two years.
Most of the flaws were cataloged as vulnerabilities and 17 obtained new CVE IDs, all of which was publicly disclosed at the RVD~\cite{vilches2019introducing}.
In most cases, these robots present few or no security measures, allowing adversaries to easily exploit the flaws of internal components (e.g. as demonstrated in  \href{https://github.com/aliasrobotics/RVD/issues/2558}{RVD\#2558}, \href{https://github.com/aliasrobotics/RVD/issues/2561}{RVD\#2561} or  \href{https://github.com/aliasrobotics/RVD/issues/2562}{RVD\#2562}), so compromising the robot behavior or taking full control of it.

We argue that robot teardown is key for security research, as proper knowledge of the hardware helps determine potential attack vectors and which additional elements can help mitigate security issues when the manufacturer does not react. As an example, our group introduced an additional commercial off-the-shelf hardware firewall within MiR's internal network between the main controller and the SICK's safety PLC mitigating \href{https://github.com/aliasrobotics/RVD/issues/2558}{RVD\#2558}, without having to modify any parts of the firmware.

Throughout this work, we found planned obsolescence particularly evident in the robots from Universal Robots. From an electrical point of view, these two robots present a similar layout for interfacing with the robot arm. The manufacturer however introduced subtle changes meant to make this particular intent harder. Our work showed how through teardown, we learned how to bypass these limitations using commercial off-the-shelf components with a total BOM price under 30 Euros.


\vspace{-0.5em}

\section{Conclusions}
We are concerned about the growing trend in robotics to create private networks of \emph{certified} groups, a common practice shown by manufacturers like MiR or UR, both owned by Teradyne. We presented robot teardowns as an approach to study robot hardware architectures, obtain repairing capabilities, uncover planned obsolescence, and research its security. We advocate for a `\emph{Right to Repair}' in robotics and encourage end-users to reflect their needs into their supply chains and into the original upstream robot manufacturers.

==> sections/III.blueprints/4.devsecops.tex <==
\chapter{DevSecOps in Robotics}
\label{chapter:devsecops}

\epigraph{\textbf{Contributions}: \emph{Leading author of \cite{mayoral2020devsecops}. Got contributions from third parties concerning editing and final content polishing. This work is in-use by various robotic companies today.}}{}

% DevSecOps + Cybersecurity in Robotics: Challenges, etc.

\section{Introduction}

\begin{figure}[h!]
    %\includegraphics[width=0.9\textwidth]{figures/secdevops_bad.png}
    %\includegraphics[width=0.9\textwidth]{figures/grafico-new.jpg}
    \includegraphics[width=0.8\textwidth]{figures/DevOps.png}
    \centering
    \caption{The DevOps cycle and its four phases: a) development, b) deployment, c) production and d) post-production}
    \label{fig:devops_cycle}
\end{figure}

Where waterfall development once dictated the process of "handing off" from developers to Quality Assurance (QA) to operations, these responsibilities now have blurred borders with most engineers’ skill sets spanning multiple disciplines. Enter \textbf{DevOps}, a set of practices that combine software development (Dev) with Information Technology operations (Ops). They aim to shorten the development life cycle and provide continuous delivery while ensuring the quality of the software (Quality Assurance or QA)\cite{ebert2016devops}. Most sources \cite{devopsorigin1, devopsorigin2} agree that this idea began around 2008, with a discussion between Patrick Debois and Andrew Clay Shafer, concerning the concept of agile infrastructure. According to Roche \cite{roche2013adopting}, no standard definition exists for DevOps. What seems clear is that the design phase has been replaced by a less cyclic and more integrated flow evolution from development to demonstrations. \\
\newline
In Robotics, as in many other areas closely connected to Computer Science, there is a set of adopted common practices, including DevOps. Figure \ref{fig:devops_cycle} pictures the DevOps cycle most roboticists use and split into 4 phases: Development, Deployment, Production and Post-Production. In the DevOps philosophy, these phases are all connected in a continuous, never-ending, loop. The waterfall is now a river; development and operations flow together but, where is security in such a landscape? As pointed out by the UK's National Cyber Security Center \cite{ncsc_uk}, having a secure approach to development has never been so critical, when it comes to cyberphysical systems and, of course, robotics. The way roboticists build software and systems is rapidly evolving, becoming more and more automated and integrated. Many roboticists today define, prototype and develop an entire robotics system architecture in simulation and tie it to tooling which will automate both testing and deployment.\\
\newline
Over the last couple of years we have seen big changes on the arrival of cloud services to robotics and to 'robot infrastructure as a service' including simulation, fleet management systems, or teleoperation capabilities among others. The promise is that robots of almost any size and complexity can be called into virtual life, changed, or terminated without leaving the desktop. On top of these new capabilities, a process of quick and regular deployments has evolved. Often referred to as Continuous Delivery, this iterative approach is powerful, flexible and efficient, but these strengths bring new sets of risks which your security practices must address. To do so, roboticists will need to consider security as a primary concern throughout your development and deployment processes. \\
\newline
To the best of the author's knowledge, while there is some prior work studying DevOps in the embedded systems field \cite{lwakatare2016towards}, there is no literature available to date formalizing the adoption of DevSecOps in the robotics domain. In this chapter we introduce DevSecOps in Robotics as a set of best practices designed to help roboticists implant security deep in the heart of their development and operations processes. The content provided below is not an in-depth guidance on how to avoid implementation vulnerabilities in the code you write, this topic is covered by other pieces of research for which the reader is kindly referred to \cite{graff2003secure, seacord2008cert, jones2004secure, seacord2005secure}. The principles provided in this chapter are intended to help secure the entire process of software development in robotics, from establishing a security-friendly culture in your organisation through implementation and ongoing management. It must be noted, however, that \emph{using these principles do not guarantee a secure final robot}, but should help you gain confidence and insights that the code you deploy is built with a security mindset.

%\todo{Speak about Quality, security and the origins of DevOps versus the waterfall model from recent article. Consider moving here the devops tihng.}


\section{From DevOps to DevSecOps}

Roche \cite{roche2013adopting} argues that developers work mostly on code while operations people work mostly with systems. Security, well identified as a continuous process, needs to be applied individually to each one of these phases and then holistically to the complete system. Security is a challenge and with each interface, the complexity increases.\\
\newline
DevOps is presented with a mix of the two skill sets mentioned above, developers and operations people. When adding security to the DevOps tuple we dive into DevSecOps. Often times called "Rugged DevOps" or “security at speed”,  \textbf{DevSecOps} is a set of best practices designed to help organizations implant security deep in their DevOps development and operations processes \cite{bird2016devopssec, mohan2016secdevops}. DevSecOps, also known as SecDevOps and DevOpsSec, seeks to embed security inside the development process as deeply as DevOps does with operations. \\
\newline
Turning again into robotics, security --identified as a process that needs to be continuously assessed both in hardware and software-- is a highly time and resource-consuming task. As was proven before in Computer Science, including security --across the development, deployment, production, and post-production phases-- results in a more secure output. Figure \ref{fig:devsecops_diagram} depicts the view on how DevSecOps could be implemented in robotics. Phases are listed as well as, tasks, and activities while providing descriptions to further clarify the effort required.


\begin{figure}[h!]
    %\includegraphics[width=0.9\textwidth]{figures/secdevops_bad.png}
    %\includegraphics[width=0.9\textwidth]{figures/grafico-2.png}
    %\includegraphics[width=0.9\textwidth]{figures/DevOps-01.jpg}
    %\includegraphics[width=0.9\textwidth]{figures/devsecops_diagram.png}
    \includegraphics[width=0.9\textwidth]{figures/devsecops_diagram.png}
    \centering
    \caption{A flowchart of DevSecOps for robotics}
    \label{figure:devsecops}
\end{figure}


\subsection{Development \emph{phase}}
\subsubsection{Plan \emph{task}}
\begin{itemize}
    \item \textbf{\bf Threat modeling}: Threat modeling is the use of abstractions to aid in thinking about risks. A threat model identifies security threats that apply to the robot and/or its components (both software and hardware) while providing means to address or mitigate them in the context of a use case and ideally, during development.
    
    \item \textbf{\bf Quality Assurance requirements}: Quality Assurance (QA) requirements imply capturing the quality metrics and aspects that will be later used to measure a code’s compliance. The requirements captured in this activity are later translated into actionable tests.

    \item \textbf{\bf Unit, integration and functional tests}: Unit testing is the practice of testing small pieces of code, typically individual functions, alone and in an isolated manner. Integration testing involves checking whether different modules perform when combined together as a group.  Finally, functional testing verifies the functionality of a given software composition, that is to confirm that the corresponding source code provides the expected behavior. In line with Test-Driven Development and other groups' practices \cite{apexaisafealgs}, it is encouraged to write tests before coding. Particularly, we encourage to a) write the general code skeleton, classes, and public methods and to b) write the test cases for the logic to implement\footnote{Note that these tests should fail at this point}.
\end{itemize}

\subsubsection{Code \emph{task}}
\begin{itemize}
    \item \textbf{\bf IDE checks}: Many vulnerabilities in products and systems could be avoided if better, more secure coding practices were in place. A number  of  Integrated  Development  Environment  (IDE) plugins exist, which help developers check for security flaws while they code \cite{basetposter}.

    \item \textbf{\bf Peer code review}: Peer Code Review, is the act of consciously and systematically analyzing fellow programmers’ code to check each other’s mistakes. Bosu et al. produced two interesting studies \cite{bosu2013peer, bosu2014characteristics} that researched vulnerabilities in code-while-in-development where they concluded that: a) the most experienced contributors authored the majority of the Vulnerable Code Changes (VCCs), b) Less experienced authors wrote fewer VCCs, but their code changes were 1.5 to 8 times more likely to be vulnerable, and c) employees of organizations sponsoring OSS (Open Source Software) projects were more likely to write VCCs. Coherently, peer code review is identified as an effective improvement practice for reducing security vulnerabilities. 
\end{itemize}

\subsubsection{Build \emph{task}}
\begin{itemize}
    \item \textbf{\bf Software Component Analysis (SCA)}: Software Component (or Composition) Analysis (SCA) is the process of identifying potential areas of risk from the use of third-party and open-source software components. In robotics, this could be very easily extended to hardware as well. SCA generally involves using a variety of different tools.
    \item \textbf{\bf Static Application Security Testing (SAST)}: Static Application Security Testing, or static analysis, is the study of software without executing it and by simply looking at its structure and content. SAST is a testing methodology that analyzes source code to find security vulnerabilities.
    \item \textbf{\bf Alert on high-risk code changes}: As a general recommendation, when the delta of code changes is above a certain pre-defined boundary, alerts should be generated.
    \item \textbf{\bf Build (compilation) checks}: CI systems generally involve one or more building process. Compilation output can deliver valuable input and should be accounted for. It is good practice to monitor a compiler’s output and file tickets for review in the warnings that remain. This can be easily automated and tickets can be filed to a centralized flaw management system like the Robot Vulnerability Database (RVD) \cite{vilches2019introducing}. An open prototype of such a flaw management system, integrated with Github, is available at \url{https://github.com/aliasrobotics/RVD} including the necessary  tooling to manage it.
\end{itemize}

\subsubsection{Test and simulate \emph{task}}
\begin{itemize}
    \item \textbf{\bf Dynamic Application Security Testing (DAST)}:  Dynamic Application Security Testing (DAST) is a practice to detect conditions indicative of a security vulnerability in an application or software in its running state. The software is tested from the outside, that is, no access to the source code is assumed to be provided and thereby falls into the black-box security testing methodologies (against SAST, which requires access to the source code and is thereby considered a white-box security testing methodology). 
    \item \textbf{\bf Deep Static Application Security Testing (Deep SAST)}: Past studies have shown \cite{barstad2014predicting, russell2018automated, gupta2018intelligent, pradel2018deepbugs} that it is possible to predict both code quality and security flaws using machine learning approaches. Deep Static Application Security Testing (Deep SAST) leverages on the the effectiveness of using machine learning-based static analysis to predict security flaws.
    \item \textbf{\bf Fuzz testing}: Fuzz testing or fuzzing, is a semi-automated testing technique for software that consists of injecting data in search for errors. It involves providing invalid, unexpected, or random data as input. The software is then monitored for exceptions such as crashes, failing code assertions, or potential memory leaks. Similar to DAST, fuzzing is a black-box security testing methodology (no access to the source code).
    \item \textbf{\bf Penetration Testing (PT or pentesting)}: Penetration testing or pentesting, is the practice of simulating a cyber attack against a given system (with a well defined scope) to check for exploitable vulnerabilities and determining its severity. Pentesting aims to find as many vulnerabilities and configuration issues as possible, in the time allotted, to then try exploit those to determine the risk of the vulnerability. A pentesting activity can be conducted as a white-box activity (complete access to source code), black-box (no access to sources or prior knowledge of the system) or gray-box (limited knowledge of the system available). Some penetration testing schemes are applicable to robotics, such as Robot Security Framework \cite{vilches2018introducing}.
\end{itemize}

\subsubsection{Flaw management \emph{task}}
\begin{itemize}
    \item \textbf{\bf Flaw management activity}: Formally \cite{foreman2019vulnerability}, flaw management is the cyclical practice of identifying, classifying, re-mediating, and mitigating flaws. Flaw management is at the center of security activity. It refers to the process of how security researchers, suppliers, and end user organizations manage bugs and vulnerabilities, making systems more secure. \\
    \newline
    Flaw management requires a holistic, risk-based approach to security and combines the input received from other phases and tasks in the security process (e.g. SAST, DAST, build warnings, pentesting, fuzzing, etc.). The amount of flaws is often bigger than the engineering resources to manage them, thereby flaws should be prioritized. This is often done using a preliminary risk assessment, which is typically performed by using severity scoring mechanisms such as CVSS \cite{mell2006common} or RVSS \cite{vilches2018towards}, the latter more specific for robotics and accounting for safety hazards. 
\end{itemize}

\subsection{Deployment \emph{phase}}
\begin{itemize}
    \item \textbf{\bf Configuration and system integration task}: Deals with system integration and configuration of all parts previously developed and conforming the robotic system. It is one of the most sensitive tasks from a security perspective. It is critical to define secure deployment mechanisms and employ strong systematic configuration practices to ensure no flaws are presented during this task.
\end{itemize}

\subsection{Production \emph{phase}}
\begin{itemize}
    \item \textbf{\bf Monitor}: This task deals with the continuous monitoring of the system and should oversee the systems' performance, errors, and other relevant information. A common good practice is to employ elements that record all activity, securely, for potential future forensics research.
\end{itemize}

\subsection{Post-production \emph{phase}}
\subsubsection*{Analyze \emph{task}}
\begin{itemize}
    \item \textbf{\bf Vulnerability Scans}: Vulnerability scans provide results on new vulnerabilities affecting your system and provides solid data on their levels of severity. This data should be fed into the Flaw Management system and prioritized based on common scoring mechanisms.
    \item \textbf{\bf Red Teaming}: Red teaming is a full-scope, holistic, multi-layered, and targeted (specific goals) attack simulation designed to measure how well a company’s systems, people, networks, and physical security controls can withstand an attack. Opposed to Penetration Testing, a red teaming activity does not seek to find as many vulnerabilities as possible to risk-assess them, instead it has a specific goal to look for vulnerabilities that will maximize damage and meet the goal. The ultimate objective of a red teaming activity is to test  organization/system detection and response capabilities in production. 
    \item \textbf{\bf Bug Bounties}: A Bug Bounty program is a coordinated and well scoped effort to encourage security research in a particular system rewarding (with bounties) those researchers who help find bugs. Bug Bounty programs utilize a pay for results model, favour competition and often leverage the crowd sourced model. Bug bounty programs can be self hosted or coordinated by third parties. There are several online providers that offer support organizing the programs. When compared to other actions such as red teaming, bug bounty programs are generally result-oriented and add more diversity on the testers side (crowd-sourcing). On the down side, bug bounty programs do not generally have highly skilled security researchers and they require extensive program management (either on you or hired).
\end{itemize}


\noindent Figure \ref{fig:devsecops_cycle} presents a graphical representation of the DevSecOps cycle in the robotics domain.

\begin{figure}[h!]
    %\includegraphics[width=0.9\textwidth]{figures/secdevops_bad.png}
    %\includegraphics[width=0.9\textwidth]{figures/grafico-new.jpg}
    %\includegraphics[width=0.8\textwidth]{figures/DevOps-01.jpg}
    \includegraphics[width=0.8\textwidth]{figures/DevSecOps.png}
    \centering
    \caption{A graphical representation of the DevSecOps cycle for robotics.}
    \label{fig:devsecops_cycle}
\end{figure}

 %===============================================================================

%\section{Security, quality and safety}
\section{Conclusion}

With DevOps, engineering efforts now serve multiple masters. Where the focus used to be purely on precision, now longevity, scalability and security (with DevSecOps) hold equal footing in product requirement discussions. Where Quality Assurance (QA) had traditionally held the line on risk definition and maintainability, Security now has an equal, if not dominant, role.\\
\newline
\textbf{Quality} (Quality Assurance or QA for short) and \textbf{Security} are often misunderstood when it comes to software. Ivers argues \cite{ivers_2017} that quality "essentially means that the software will execute according to its design and purpose" while "security means that the software will not put data or computing systems at risk of unauthorized access". Within \cite{ivers_2017} one relevant open question that arises is whether the quality problems are also security issues or vice versa. Ivers indicates that quality bugs can turn into security ones, provided they are exploitable, and addresses the question by remarking that quality and security are critical components to a broader notion: software integrity. Coming from the same group, Vamosi \cite{vamosi_2017} argues that "quality code may not always be secure, but secure code must always be quality code". This somehow conflicts with the previous view and leads one to think that secure software is a subset of quality. This chapter reject this view and argue instead that Quality and Security remain two separate properties of software that may intersect on certain aspects (e.g. testing). This topic is discussed in more detail in chapter \ref{chapter:background}.\\
\newline
As nicely indicated by Lopez \cite{lopez_2017} for the DevOps scenario and extending it for security, in the DevSecOps scenario, both security and QA integrate into the testing and development processes and take a collaborative approach. Quality and Security are ensured throughout the testing and delivery cycles and both the testing and development teams are responsible for them. In other words, \emph{compared to the traditional waterfall pattern where quality creeps in toward the end, with DevSecOps security and quality come in at every level}.
\newline
In robotics there is a clear separation between Security and Quality that is best understood with scenarios involving robotic software components. For example, if one was building an industrial Automated Guided Vehicle (AGV), Autonomous Mobile Robots (AMRs) or a self-driving vehicle, often, she/he would need to comply with coding standards (e.g. MISRA \cite{ward2006misra} for developing safety-critical systems).  The same system's communications, however, regardless of its compliance with the coding standards, might rely on a channel that does not provide encryption or authentication and is thereby subject to eavesdropping and man-in-the-middle attacks. Security would be a strong driver here and as remarked by Vamosi \cite{ivers_2017}, "neither security nor quality would be mutually exclusive, there will be elements of both".\\
\newline
Quality in robotics, still on its early stages \cite{pichler2019can} (though much more developed than security in the author's opinion), is often viewed as a pre-condition for \textbf{Safety}-critical systems. Similarly, as argued by several, safety can not be guaranteed without security \cite{goertzel2009software, bagnara2017misra}. Coding standards such as MISRA C have been extended \cite{misra2016amendment1, misra2016addendum2} to become the "C coding standard" of choice for the automotive industry and for all industries developing embedded systems that are safety-critical and/or security-critical \cite{bagnara2017misra}. As introduced by ISO/IEC TS 17961:2013 "in practice, security-critical and safety-critical code have the same requirements". This statement is somehow supported by Goertzel \cite{goertzel2009software} but emphasized the importance of software remaining dependable under extraordinary conditions and the interconnection between safety and security in software. This same argument was later extended by Bagnara \cite{bagnara2017misra} who acknowledges that having embedded systems, non-isolated anymore, plays a key role in the relationship between safety and security. According to Bagnara, "while safety and security are distinct concepts, when it comes to connected software" (non-isolated)  "not having one implies not having the other", referring to integrity.\\
\newline
Acknowledging that both Security and QA are embed into the DevSecOps cycle brings us to question whether safety --connected to Quality-- could also fit in. Myklebust et al. \cite{myklebust2019safety} argue that DevOps, with its frequent changes, make systems’ maintainability – e.g., change impact analysis – a more challenging topic, which makes it more difficult to integrate safety within the DevOps cycle. They do acknowledge though that DevOps is also a considerable trend for non-critical systems and make an interesting connection between safety and security, which indirectly leads to DevSecOps. In a similar line of thought, Johnson \cite{johnson_2018_performance} indicates that the time and cost involved in this process makes the DevOps paradigm of continuous release challenging for safety-critical software, especially in delivering to the end customer. He, however, points out that despite this, "aviation and defense teams have embraced the principles of DevOps, especially at the pre-certification stage, because of the potential for the higher overall quality it offers".\\
\newline
Altogether this leads us to the following questions: how do we apply safety-critical practices to the DevSecOps cycle in robotics? And more importantly, if safety and security coding (software) standards do not guarantee that the final robotic system will be secure, will it be safe given the safety and security connection? Some preliminary work \cite{meyers2019model, di2016software} tackles the first question and indicates that Model-Driven Engineering (MDE) frameworks might allow a mix of DevSecOps with the functional safety process. The work presented in this chapter establishes a set of best practices designed to help roboticists implant security into their robot development and operations processes. Such practices can easily be translated into an MDE framework which then guide roboticists in their design tasks. Further research on this line of work and on some of  these questions remain open for future efforts.


==> sections/III.blueprints/8.tools.tex <==
\chapter{Tools for Robot Cybersecurity}
\label{chapter:tools}

\epigraph{\textbf{Contributions}: \emph{Leading author and source code contributor at \cite{mayoral2023exploitflow} and \cite{mayoral2020alurity}. ExploitFlow is open source. Alurity is proprietary and used in day-to-day security operations.}}{}


Building on the insights gained in the previous chapters about defensive security approaches for robots including DevSecOps (chapter \ref{chapter:devsecops}), ROS 2 security mechanisms and tools (chapter \ref{chapter:ros_security}), benchmarking the computational security overhead (\ref{chapter:benchmarking}) and hardware accelerators to speed up critical computations in robotics (\ref{chapter:accelerators}), this chapter shifts focus from a defensive to an offensive approach in robot security. We introduce and discuss two pivotal tools, Alurity and ExploitFlow, designed to advance offensive security research and measures in robotics. These tools represent a significant stride in addressing and mitigating security threats, enabling researchers and practitioners to proactively identify, research and exploit vulnerabilities within robotic systems. Their development and application signify a critical step in comprehensively strengthening the security posture of robotic systems.

% Alurity
% ExploitFlow

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Alurity}
\showkeysfalse  % Disable keys    
\label{tools:alurity}
\showkeystrue  % Enable keys    


\subsection{Introduction}

% TODO:
% - Introduce bits from PhD thesis on the difficulties of robot cybersecurity
% - Introduce bits from SOTA research
% - Introduce bits alurity documentation

Cybersecurity is not a product, but a process. One that needs to be continuously assessed in a periodic manner, as systems evolve and new cyber-threats are discovered. This becomes specially relevant with the re-use of (software and hardware) components and the increasing complexity of such systems \cite{bozic2017planning}. Robotics is the art of system integration \cite{mayoral2017shift}. Its modular characteristic by nature, both in hardware and software, provides unlimited flexibility to its system designers. This flexibility however comes at the cost of increased complexity. Current robotic systems are often highly complex, a condition that in most cases leads to wide attack surfaces and a variety of potential vulnerabilities, which increase the complexity of remaining secure by solely relying on the use of traditional perimeter-based approaches. 

Robot cybersecurity vulnerabilities are potential attack points in robotic systems that can lead not only to considerable loss of data, but also to safety incidents involving humans \cite{kirschgens2018robot}. Some claim \cite{zheng2011ivda} that unresolved vulnerabilities are the main cause of loss in cyber-incidents. Given the interaction robots have with humans and our environments, the qualification of a security flaw, commonly known as \emph{triage}, seems of special relevance in the domain of robotics. Mitigating a vulnerability or a bug often requires one to first triage and reproduce the flaw in a  deterministic manner. 
%From the authors’ experiences and involvement in the construction of robotic systems, working with robots is generally very time consuming.
Dealing with robots requires interacting with both hardware and software. The strong interdisciplinary of the robotics fields (which is an inherent characteristic of the complexity of the area) and the trade-off obtained with its modularity~\cite{Kolak2020ItTakesAVillage} demands for knowledge across multiple domains in order to comprehensively analyze a robot system. Correspondingly, triaging and reproducing security flaws in robotics can become extremely demanding in terms of time and resources, especially when cooperating with team members across multiple locations, several of which don't necessarily may have access to the same hardware. 

To address this and accelerate research, a toolbox for robot cybersecurity should facilitate the creation of virtual environments that capture not only software components, but also hardware ones. OS-virtualization and hardware-virtualization are both needed in robotics, specially with the growing adoption of modular frameworks like the Robot Operating System (ROS) \cite{quigley2009ros}. We believe that emulation and simulation should co-exist for robot cybersecurity research, and it should be possible to easily interface these with real hardware.


The present section attempts to deal with these problems by proposing a cybersecurity toolbox that aims to enable roboticists and security researchers cooperating in project to have a common, consistent and easily reproducible development environment, facilitating the security process (DevSecOps \cite{mayoral2020devsecops}) in robotics and the collaboration across multiple teams. The contributions of this work are threefold. First, we present a modular toolbox for robot cybersecurity that facilitates the cybersecurity processes. It reflects the modular nature of robotics while at the same time makes the resulting complexity easier to handle for cybersecurity researchers. Second, we demonstrate support for mixed simulation and emulation environments in robotics. This helps research  scenarios involving high-fidelity virtual versions of hardware and software robot components. Finally, through composability, the toolbox provides modules that can be selected and assembled in various combinations, providing facilities for automation of security testing, evaluation and demonstration while enhancing the triage and reproducibility of security flaws.


%The remaining content is organized as follows: Section \ref{sec:background} presents previous related work. Section \ref{sec:alurity} describes the toolbox and section \ref{sec:use_cases} a series of use case experiences. Section \ref{sec:lessons_learned} presents results using the toolbox and argues about some of the lessons learned throughout the process. Finally, Section \ref{sec:conclusions} summarizes our work and draws some conclusions while hinting on future work actions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BACKGROUND
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Background}


\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.4}
\begin{table*}[h!]
    \centering
	\resizebox{\textwidth}{!}{ 
		\begin{tabular}{|l|l|l|l|l|l|l|l|}
			\hline
            \rowcolor{black}
			& \color{white}\bf \textsc{Scope} & \color{white}\bf \textsc{Simulation} & \color{white}\bf \textsc{Emulation} & \color{white}\bf \textsc{Mixed} & \color{white}\bf \textsc{Scalable} & \color{white}\bf \textsc{Flexible}  \\ 
			\hline
			DETERlab~\cite{5655108} & testbed facility, hardware testing &  \cellcolor{black!15} No  & Yes  & \cellcolor{black!15} No  & \cellcolor{black!15} Low      & Yes\\ 
			%\hline
			VINE~\cite{Eskridge:2015:VCE:2808475.2808486} & computer networks, dynamic and moving target defenses  & \cellcolor{black!15} No         & Yes       & \cellcolor{black!15} No  & \cellcolor{black!10} Med      & Yes\\ 
			%\hline
			SmallWorld~\cite{FURFARO2018791} & computer networks, network devices, hardware devices  & \cellcolor{black!15} No         & Yes       & \cellcolor{black!15} No  & \cellcolor{black!10} Med      & Yes\\ 
			%\hline
			BRAWL~\cite{BRAWL} & enterprise computer networks & \cellcolor{black!15} No         & Yes       & \cellcolor{black!15} No  & \cellcolor{black!10} Med      & \cellcolor{black!15} Windows \\ 
			%\hline
			Galaxy~\cite{schoonover2018galaxy} & computer networks & \cellcolor{black!15} No         & Yes       &  \cellcolor{black!15} No  &  \cellcolor{black!15} Low      & \cellcolor{black!15} Debian-based\\ 
			%\hline
			Insight~\cite{Futoransky2009SimulatingCF} & computer networks, network devices, hardware devices & Yes        & \cellcolor{black!15} No        & \cellcolor{black!15} No  & High     & Yes\\ 
			%\hline
			CANDLES~\cite{Rush:2015:CAN:2739482.2768429} & computer networks, game theory & Yes        & \cellcolor{black!15} No        & \cellcolor{black!15} No  & High     & Yes\\ 
			%\hline
			Pentesting Simulations~\cite{niculae_2018, JThesis} & computer networks, penetration testing, machine learning  &  Yes        & \cellcolor{black!15} No        & \cellcolor{black!15} No  & High     & Yes\\ 
			%\hline
			CyAMS~\cite{7795375} & computer networks, malware propagation & Yes & Yes  & \cellcolor{black!15} No  & High     & Yes\\ 
			%\hline
			CybORG~\cite{baillie2020cyborg} & computer networks, machine learning &  Yes        &  Yes       &  \cellcolor{black!15} No  &  High     & Yes\\ 
			%\hline
			%\rowcolor{black!15} % ours
			\bf \emph{alurity} (ours) & \bf robotics, industrial devices, computer networks & \bf Yes        &  \bf Yes       &  \bf Yes  &  \bf High     &  \bf Yes\\ 
			\hline
		\end{tabular}
	}
	\caption{A comparison of cybersecurity-focused environments and frameworks.} 
 %Each one of them is evaluated according to five characteristics: simulation capabilities, emulation capabilities, mixed simulation and emulation capabilities, scalability (complex environments, multiple endpoints, etc.) and flexibility in terms of the requirements to run it. With regard the mixed column, note it refers to either the presence of both (emulation and simulation) as complete entities in an scenario, or alternatively the possibility to simulate some parts, and emulate others both together in a combined entity.}}
	\label{table:cybersecurity_virtualization}
\end{table*}


The mitigation and patching of vulnerabilities has been an active area of research \cite{ma2001sharing, ALHAZMI2007219, Shin2011Vulnerabilities, Finifter2013BugBounty, McQueen2009Zeroday, Bilge:2012:BWK:2382196.2382284} in computer science and other technological domains. Unfortunately, with robotics being an interdisciplinary field composed from a set of heterogeneous disciplines (including computer science), to the best of our knowledge and literature review, except for a few preliminary tools and reviews \cite{mayoralrvd, vilches2018towards, ekenna2020clustering, mayoral2020can, dieber2020penetration, lacava2020current}, not much vulnerability mitigation research related to robotics has been presented so far.

Due to their expensive prices and shortage, getting access to robots for testing is somewhat comparable to the difficulties researchers face when analyzing complex computer networking systems. The Galaxy framework~\cite{schoonover2018galaxy} researched this and proposed a high-fidelity computer network emulation tool designed to support rapid, parallel experimentation with the automated design of software agents in mind. By leveraging virtualization, the authors of Galaxy create a high-fidelity clone of a network that takes snapshots to always have a copy of this known base state. With this cloned network, researchers can distribute the work and perform experiments to see how the network performs with certain kind of attacks. 

Virtualization is a commonly used technique in other areas allowing developers and security practitioners to more easily test, reuse and ship systems. When using virtualization, there are often two approaches, emulation and simulation. Emulation is generally implemented through hardware-virtualization, typically using full-virtualization with type two hypervisors (e.g. VirtualBox, VMWare Worksation or QEMU) \cite{grattafiori2016understanding}, commonly referred to as Virtual Machines (VMs). This provides complete isolation between guest kernels and host, while allowing to run many different operating Systems (OS) within the same physical host. Simulation is often implemented with simpler abstractions such as state machines or through OS-virtualization, using a shared kernel across both the host and guests. OS-virtualization is typically referred to as "containers" in Linux \cite{grattafiori2016understanding}, and is widely considered the most efficient virtualization method for its highest performance and fastest "start-up" time. Different approaches to simulation are presented at \cite{Futoransky2009SimulatingCF, Rush:2015:CAN:2739482.2768429, niculae_2018, JThesis, 7795375, baillie2020cyborg}.

The authors of \cite{schoonover2018galaxy} confirm that shifting from simulated to emulated experiments removed the luxury of real-world abstractions and acknowledge that VMs must be power cycled, or reverted to reset states, as opposed to quicker simulations. They further mention that VM emulation is bulky and computationally expensive, whereas containers (OS-virtualization) use fewer system resources and have faster power cycle actions. A concerning matter regarding OS-virtualization is that unlike VMs, which emulate the entire network architecture stack, containers share the host kernel which comes at the cost of fidelity. This was raised by \cite{schoonover2018galaxy} however Handigol et al. \cite{handigol2012reproducible} and Heller \cite{heller2013reproducible} demonstrated how containers, could be used without a relevant loss of fidelity, which further encourages the use of containerization. Other approaches to emulation include \cite{5655108, Eskridge:2015:VCE:2808475.2808486, FURFARO2018791, BRAWL, 7795375} or \cite{baillie2020cyborg}.

A similar experience to \cite{schoonover2018galaxy} was described more recently by \cite{baillie2020cyborg} which targets research in Autonomous Cyber Operations (ACO). The authors of \cite{baillie2020cyborg} proposed a high-fidelity emulation using VMs, and a low-fidelity simulation using a finite state machine design that could model networks. Virtualization of the different scenarios was realized by using a description file (YAML) and a flag determined the use of either simulation or emulation. The results obtained of this dual approach show promise and the authors already hint that future work might train in low-fidelity simulation, and later optimize in high-fidelity emulation.

%Finally, ACO environments have high complexity and dimensionality, with very many interdependent and related components and large state

Our work builds on top of these past experiences and proposes a toolbox that facilitates the virtualization of robotic scenarios with the capability of doing both high-fidelity emulation and simulation using VMs and containers, respectively. Moreover, by extending the networking abstractions of both VMs and containers, our toolbox allows for mixed heterogeneous virtual environments, where emulated endpoints (VMs) can interact with simulated ones (containers), providing more flexibility for roboticists and security researchers. Table \ref{table:cybersecurity_virtualization} presents our approach compared to past work. Each one of them is evaluated according to five characteristics: simulation capabilities, emulation capabilities, mixed simulation and emulation capabilities, scalability (complex environments, multiple endpoints, etc.) and flexibility in terms of the requirements to run it. With regard the mixed column, note it refers to either the presence of both (emulation and simulation) as complete entities in an scenario, or alternatively the possibility to simulate some parts, and emulate others both together in a combined entity.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALURITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The tool: alurity}


\emph{Alurity} is a modular and composable toolbox for robot cybersecurity. It ensures that both roboticists and security researchers working on a project, have a common, consistent and easily reproducible development environment facilitating the security process and the collaboration across teams. It's available for Linux (across distributions) and Mac OS, with limited support at the time of writing for Windows. Featuring dozens of different tools in the form of individual components, \emph{alurity} simplifies and speeds up the cybersecurity research in robotics. The toolbox organizes security and robotics components in different groups that allow for easy composition and use. Figure \ref{figure:alurity_toolbox} illustrates this aspect and the different groups, while constructing a robotic subject with it. The toolbox classifies tools in seven groups that favour composition and re-usability among them. The groups are: robots, robot components, forensics, exploitation, testing, reconnaissance and IDE/UI. In the left, we depict a subset of the tools available, across the different groups. The right hand side illustrates a composition of tools into a construction that will be used during the robot cybersecurity research effort. The subject constructed features a base ROS \cite{quigley2009ros} module, and a number of submodules composed below including the UR3 ROS driver, the MoveIt \cite{chitta2012moveit} Motion Planning Framework ROS packages, the aztarna \cite{vilches2018aztarna} footprinting tool for robots, the Gazebo \cite{koenig2004design} robot simulator or robosploit, a proprietary exploitation framework for robots, among others.

Similar to \cite{baillie2020cyborg}, \emph{alurity} toolbox allows to build scenarios using a simple description file in YAML format. Listing \ref{alurity:example} provides an example of such format while modeling the scenario of Figure \ref{figure:alurity_use_cases:ur}.

\lstset{morekeywords={network, networks, name, driver, internal, encryption, subnet, ip, firewalls, container, ingress, egress, rules, modules, base, cpus, memory, mount, volume}}
\lstset{label={alurity:example}}
\lstset{basicstyle=\tiny,
    numbers=none,
    firstnumber=1,
    stepnumber=1}
\lstset{caption={
    \footnotesize \emph{Alurity} YAML syntax to simulate a UR3 controller and an attacker, as part of the use case depicted in Figure \ref{figure:alurity_use_cases:ur}.}
}
\begin{lstlisting}
networks:
  - network:
    - name: process-network
    - driver: overlay
    - internal: true
    - encryption: false
    - subnet: 12.0.0.0/24

  - network:
    - name: cloud-network
    - driver: overlay
    - subnet: 17.0.0.0/24
    
containers:
  - container:
    - name: "ur3"
    - modules:
         - base: registry.gitlab.com/aliasrobotics/offensive/alurity/robo_ur_cb3_1:3.13.0
         - network:
           - process-network
    - ip: 12.0.0.20  # assign manually an ip address
    - cpus: 4
    - memory: 2048

  - container:
    - name: attacker
    - modules:
         - base: registry.gitlab.com/aliasrobotics/offensive/alurity/comp_ros:melodic-scenario
         - volume: registry.gitlab.com/aliasrobotics/offensive/alurity/expl_robosploit/expl_robosploit:latest
         - volume: registry.gitlab.com/aliasrobotics/offensive/alurity/reco_aztarna:latest
         - volume: registry.gitlab.com/aliasrobotics/offensive/alurity/deve_gazebo:latest
         ...
         - network:
           - process-network
           - cloud-network
    - extra-options: ALL

\end{lstlisting}


\begin{figure*}[!h]
    %\includegraphics[width=1\textwidth]{figures/alurity-attack-2.png}
    \includegraphics[width=0.9\textwidth]{figures/alurity_table.pdf}
    \centering
    \caption{
        \emph{alurity} toolbox for robot cybersecurity
    }
    \label{figure:alurity_toolbox}
\end{figure*}

\subsubsection{Simulated, emulated or real endpoints}

Dealing with robots requires interacting with both hardware and software. Correspondingly, a toolbox that helps security researchers and roboticists in their cybersecurity efforts should consider virtual environments that capture not only software components, but also hardware ones. OS-virtualization and hardware-virtualization are both needed. In other words, emulation and simulation should co-exist. 

Virtualization in \emph{alurity} defaults to simulation. Built using containers (OS-virtualization) it delivers an efficient, high-fidelity, high-performance and fast virtualization method. Most \emph{alurity} modules (tools) are containerized this way and can be easily composed as demonstrated in listing \ref{alurity:example}. High-fidelity emulation is implemented using VMs (hardware-virtualization)---more specifically---on top of VirtualBox VMs (full-virtualization, type two hypervisor). The YAML syntax for emulation is similar to the one for simulation and exemplified in listing \ref{alurity:example2}:

\lstset{morekeywords={network, networks, name, driver, internal, encryption, subnet, ip, firewalls, container, ingress, egress, rules, modules, base, cpus, memory, mount, volume}}
\lstset{label={alurity:example2}}
\lstset{basicstyle=\tiny,
    numbers=none,
    firstnumber=1,
    stepnumber=1}
\lstset{caption={
    \footnotesize \emph{Alurity} YAML syntax to emulate an ABB’s IRC5 Compact robot controller as per the use case depicted in Figure \ref{figure:alurity_use_cases:abb}.}
}
\begin{lstlisting}
vms:
  - vm:
    - name: irc5
    - path: $(pwd)/vms/irc5
    - network: process-network
    - ip: 12.0.0.100
    - cpus: 2
    - memory: 2048
\end{lstlisting}



\emph{Alurity} allows to easily build robotic subjects of study through the virtualization of different robots, networks (e.g. LANs, serial comms, VPNs, VLANs, VXLANs, WLANs, etc) and robot components, including security protection mechanisms as depicted in Figure \ref{figure:alurity_use_cases:kics}. It supports both, simulation and emulation of modules and allows for mixed environments where emulated endpoints can co-exist and interact (networking-wise) with simulated ones. This logic is implemented at the core of the toolbox through private network internals to the host so that containers on this network can communicate with VMs. Behind the scenes, \emph{alurity} creates the necessary bridges, internal virtual network interfaces, iptables rules, and host routes to make this connectivity possible. 

Beyond virtualization (emulation or simulation), \emph{alurity} was built to include real robot endpoints in the scenarios. Correspondingly, the toolbox and its networking capabilities allow to interface with public networks and interoperate with real robots, while leveraging the power to build virtual attackers and weaponize them with different tools and exploits.

\subsubsection{Flows}

\emph{Alurity} operates mostly through its Command Line Interface (CLI), which facilitates to download your configuration YAML file modules and start the scenarios, to begin with the corresponding experiments. Beyond core modules, \emph{alurity} provides an additional capability called \texttt{alurity flows} meant to facilitate evidence generation and reproduction. Flows are series of commands within a scenario built with \emph{alurity}. A flow allows to automate interactions between endpoints through the launch of a series of commands and applications via simple YAML format. Simply put, flows allow researchers to reproduce each other's work and results by simply providing a YAML file with the scenario description and one (or multiple) flows. \emph{alurity} flows are built using a mix of tools including byobu, tmux and other utilities which are embed into a base layer present in every \emph{alurity} module. Listing \ref{alurity:example3} exemplifies a flow where an attacker targets the ROS core of an industrial setup. 

To further automate security research, \emph{alurity} YAML files, including the flows, can be integrated into vulnerability tickets of robot vulnerability databases, such as the Robot Vulnerability Database (RVD) \cite{mayoralrvd}, allowing other researchers to simply \texttt{alurity run --rvd <ticket-id>} fetching the corresponding \emph{alurity} YAML portion and launching its flow for reproducing the vulnerability. Examples of this include \cite{rvd2554, rvd2555, rvd2556} or \cite{rvd2558} among others.


\lstset{morekeywords={network, networks, name, driver, internal, encryption, subnet, ip, firewalls, container, ingress, egress, rules, modules, base, cpus, memory, mount, volume, window, commands, command, split, flow}}
\lstset{basicstyle=\tiny,
    numbers=none,
    firstnumber=1,
    stepnumber=1}
\lstset{caption={
    \footnotesize \emph{Alurity} YAML syntax to create a flow that launches a FIN-ACK attack against the ROS master machine ($S_7$) in the use case depicted in Figure \ref{figure:alurity_use_cases:rosi}}
}
\lstset{label={alurity:example3}}
\begin{lstlisting}
flow:
  # rosmachine
  - container:
    - name: rosmachine
    - window:
      - name: ros
      - commands:
        - command: "source /opt/ros/melodic/setup.bash"
        - command: "roscore"
        - split: horizontal
        - command: "source /opt/ros/melodic/setup.bash"
        - command: "sleep 10"
        - command: "rostopic echo /chatter"
        - split: horizontal
        - command: "source /opt/ros/melodic/setup.bash"
        - command: "sleep 10"
        - command: "rostopic hz /chatter"
        
  # attacker
  - container:
    - name: attacker
    - window:
      - name: setup
      - commands:
        - command: "wireshark -i eth0 . &"
        - split: horizontal
        - command: "apt-get update && apt-get install -y tcpdump iptables"
    - window:
      - name: attack
      - commands:
        - command: "source /opt/ros/melodic/setup.bash"
        - command: 'export ROS_MASTER_URI="http://12.0.0.2:11311"'
        - command: "cd /home/alias"
        - command: "sleep 10"  # wait until roscore is ready
        - command: "/opt/ros/melodic/lib/roscpp_tutorials/talker"
        - split: horizontal. % create a terminal split and spawns a new shell
        - command: "sleep 10"  # wait until tools have been installed and roscore
        - command: "source /opt/ros/melodic/setup.bash"
        - command: 'export ROS_MASTER_URI="http://12.0.0.2:11311"'
        - command: "cd /home/alias"
        - command: "iptables -I OUTPUT -s 12.0.0.4 -p tcp --tcp-flags RST RST -j DROP"
        - command: "iptables -I OUTPUT -s 12.0.0.4 -p tcp --tcp-flags FIN FIN -j DROP"
        - command: 'python3 fin_ack_dos.py'
        - command: 'robosploit -m exploits/ros/fin_ack -s "target 12.0.0.2"' 
    - select: attack
\end{lstlisting}


\subsubsection{Pipelines}

When performing a security exercise, researchers often spend a considerable amount of time with information gathering and testing, for bug identification. This process is often performed manually, consuming resources that could instead be used for exploitation and/or mitigation. In order to alleviate this effort we built \texttt{alurity pipelines}, automated end-to-end and on-demand security pipelines that automatically build an \emph{alurity} YAML file with selected tools and "runs them" through the desired target module. For each security flaw identified, the pipeline generates a YAML file describing the flaw using RVD \cite{mayoralrvd} taxonomy\footnote{Available at \url{https://bit.ly/36Y7uxt}} either in a local directory or pushing the flaw directly as an issue to Github or Gitlab. This way, pipelines support the robotics DevSecOps \cite{mayoral2020devsecops} pushing each potential vulnerability to a centralized flaw management registry.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use code listing instead

\begin{comment}

\begin{figure}[!h]
    \includegraphics[width=0.5\textwidth]{figures/alurity-attack-2.png}
    \centering
    \caption{\todo{
        \footnotesize \textbf{Use case architecture diagram}. The synthetic scenario presents a network segmented in 5 levels with segregation implemented following recommendations in NIST SP 800-82 and IEC 62443 family of standards. There are 6 identical robots from Universal Robots presenting a variety of networking setups and security measures, each connected to their controller. $\hat{S_n}$ and $\hat{C_n}$ denote security hardened versions of an $n$ control station or controller respectively.
    }}
    \label{fig:architecture}
\end{figure}

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% USE CASES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Use cases}
\showkeysfalse  % Disable keys    
\label{sec:use_cases}

\begin{figure}[!h]
    \centering
    %%%%%%%%%%%%%%
    % UR scenario
    %%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.8\textwidth]{figures/ur_scenario.png}
        \caption{
        \footnotesize Simulated scenario with a Universal Robots UR3 robot and a CB3.1 controller connected to a process level network where an attacker has compromised a machine.
        }
        \label{figure:alurity_use_cases:ur}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    %%%%%%%%%%%%%%
    % ABB scenario
    %%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.8\textwidth]{figures/abb_scenario.png}
        \caption{
        \footnotesize Mixed virtual and real scenario composed by an ABB’s IRC5 compact robot controller with the IRB140 Manipulator and the DSQC 679 teach pendant.
        }
        \label{figure:alurity_use_cases:abb}
    \end{subfigure}
    ~
    %%%%%%%%%%%%%%
    % KICS scenario
    %%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.8\textwidth]{figures/kics_scenario.png}
        \caption{
        \footnotesize Mixed virtual industrial factory automation process with security integrated, namely the Kaspersky Industrial CyberSecurity (KICS) solution and Alias Robotics' Robot Immune System (RIS).
        }
        \label{figure:alurity_use_cases:kics}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    %%%%%%%%%%%%%%
    % ROS-Industrial scenario
    %%%%%%%%%%%%%%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=0.8\textwidth]{figures/rosindustrial_diagram.png}
        \caption{
        \footnotesize A simulated synthetic industrial scenario powered by ROS and ROS-I packages which presents a network segmented in 5 levels with segregation implemented following security standards.
        }
        \label{figure:alurity_use_cases:rosi}
    \end{subfigure}
    \showkeystrue  % Enable keys    
    \caption{Use cases realized with \emph{alurity} toolbox.}
    \label{figure:alurity_use_cases}
\end{figure}

%Several of the authors have individually or jointly used alurity toolbox for robot cybersecurity research. We

% I must confess it is not at all clear to me when you want or should use simulation or emulation for a particular component. Nothing is discussed about that in section III.A, and in the use cases in fig 2 sometimes the hardware is simulated, sometimes it is emulated, and I really don’t understand what drives this choice. I would save some space on the YAML snippets and discuss this issue: maybe a general discussion in III.A and in use cases section maybe explain why mixed simulation and emulation was relevant for scenarios b) and c) but not for a) and d).

To illustrate the flexibility of the \emph{alurity} toolbox, Figure \ref{figure:alurity_use_cases} depicts several use cases of robot cybersecurity research conducted with it. For each one of these scenarios, either simulation and/or emulation was used, interfacing when appropriate with real hardware for final validation of the flaws. We discuss below briefly each use case and the virtualization mechanisms used:

\subsubsection{Penetration testing Universal Robots's UR series}

Using \emph{alurity}, we conducted a penetration testing security exercise with the aim of providing a practical assessment of the UR3, UR5 and UR10 robot insecurities. Before the exercise, there were five reported vulnerabilities for these collaborative robots. After the penetration testing assessment, more than 80 were publicly available, many with proof-of-concept exploits.

Figure \ref{figure:alurity_use_cases:ur} depicts the scenario we assumed for the exercise  with a Universal Robots UR3 robot and a CB3.1 controller connected to a process level network, where an attacker had compromised a machine. The scenario was simulated with \emph{alurity} and both the robot controller and the attacker were containerized. The mechanics of the robot were ignored for the purpose of the study. While emulation could have added additional fidelity to the robot controller virtualization at the expense of additional time, we decided not to proceed in that direction and instead focused mostly on simulation, with the exception of physical attack vectors, which were conducted against the real robot with an \emph{alurity} simulated attacker. Public results were discussed at \cite{pentestingur}. A complete list of the vulnerabilities released is available at \url{https://bit.ly/3183cQF}.

%Out of these use cases more than 100 vulnerabilities were identified and reported to the corresponding manufacturers, with several dozens of new CVE IDs obtained and public disclosures at RVD \cite{mayoralrvd}.


\subsubsection{Penetration testing ABB's IRC5 controller}

We studied ABB’s IRC5 compact robot controller with the IRB 140 manipulator and the DSQC 679 teach pendant. For the use case, we assumed the controller was connected to a simulated process level network where an attacker had compromised a machine. Given the closed environment of ABB's technology, in this case, we used \emph{alurity} to mix simulation, emulation and real hardware while conducting the penetration testing assessment. The Attacker was simulated, the manipulator and the teach pendant were real and the controller was either real or emulated. Emulations of the controller consisted of isolated components extracted from its firmware. Public results of the exercise were discussed at \cite{pentestingabb}. A complete list of the vulnerabilities released during the exercise conducted within 2020 for ABB is available at \url{https://bit.ly/2FsZQzX}


\subsubsection{Penetration testing KICS}

This use case considered a more sophisticated environment involving more elements and capturing a selected portion of a secure industrial factory automation process. In particular, we focused our study on how insecure robots could be used as entry points to further compromise the Kaspersky Industrial CyberSecurity (KICS) solution, a commercial product. KICS imposes strong demands on the kernel and the hardware devices available from the file system, thereby after struggling with containerization for a while, we opted for emulating KICS-related entities including KSC, KICS for Networks  and the associated sensors\footnote{Details on KICS solution is beyond the scope of this chapter.}. We used \emph{alurity} to harmonize all networking aspects of the scenario and simulate the rest of the endpoints involved including robot controllers, workstations and other ICS elements. Results of the exercise are not publicly available at the time of writing.


\subsubsection{Red teaming ROS-Industrial}
In this use case we aimed to answer the question of whether ROS could be used securely for industrial use cases. We did so experimentally by performing a targeted offensive security exercise in a use case involving ROS-Industrial and ROS packages. We built a synthetic industrial scenario which presented a network segmented in 5 levels, with segregation implemented following standardized recommendations. \emph{Alurity} was used to simulate all entities and network elements, including those necessary for segmentation and segregation. By doing so we obtained a lightweight yet high-fidelity environment whereto perform attacks. Results of the exercise are discussed at \cite{redteamingrosi} and further documented in \cite{redteamingrosindustrial_whitepaper, mayoral2020can}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LESSONS LEARNED AND RESULTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lessons learned and results}

% That said, would it make sense to ask – and perhaps answer in Section V – if alurity could also be used to *run known attacks* on *new implementations* or even *new security mechanisms*, in an attempt to empirically test their robustness? I am sort of thinking about testing new stuff for robustness against known attacks. This would sure be possible, would it? If so, it could be a nice statement in the conclusions or lessons learned, if you find that it would fit.

At the time of writing \emph{alurity} toolbox features more than 70 different modules, including security tools, industrial common endpoints (e.g. PLCs or HMIs), robots and robot components. Due to our aim to use well-tested and established technology, as opposed to reinvent the wheel on security tooling, we re-used as much past work as possible when building the toolbox. Specially on the simulation and virtualization infrastructure side which led us to save a significant amount of resources, focusing our efforts instead on a) usability and b) optimizing the delivery of cybersecurity research products, namely vulnerabilities, proof-of-concept (PoC) exploits and mitigations. Maintaining this focused attitude on re-use is what led us to produce usable cybersecurity research results. Out of the use cases in Figure \ref{figure:alurity_use_cases}, we produced several dozens of vulnerabilities and received multiple new CVE IDs while responsibly disclosing the flaws to the upstream manufacturers. Public disclosure of these vulnerabilities happened in RVD \cite{mayoralrvd} with results catalogued by manufacturer, robot or robot component\footnote{Refer to section \ref{sec:use_cases} for examples of which vulnerabilities were found}.

Thanks to the use of virtualization, a significant amount of time was saved. Research could run in parallel among researchers and across groups, with the few physical robots available used only for final validation. The use of high-fidelity simulation also accelerated the process of dynamic testing, wherein the robot often entered into unstable states. Power-booting simulations required just a few seconds (as opposed to minutes with emulated robots, or an even longer time if having to re-flash firmware in the real robot). A particular \emph{alurity} feature that simplified peer-triage was \texttt{alurity flows} which when embed into vulnerability reports (as in \cite{rvd2554} or \cite{rvd2555}) complemented nicely exploit PoCs with additional context. Another aspect of the toolbox that proved useful was to run known attacks on new firmware versions of the robots or robot components. Specially in combination with simulations described by the YAML syntax which allowed for quick changing of the targets by simply modifying only one YAML line. The same applied to new security mechanisms, which could be tested against attacks, and across robots easily with \emph{alurity}.

Overall, after these experiences and although we don't feel we could generalize for all use cases, we strongly recommend security researchers to consider testing and triaging in simulation before defaulting to emulation and ultimately, to real endpoints. This will save them a considerable amount of time and will facilitate reproduction and interactions with upstream vendors, who are likely the final recipients of their security results.

% lots of small experiments which make YAML sometimes cumbersome, creation of "alurity run" verb to make quick interations in simulation with one or several modules. In addition, YAML format was extended to include syntax that automatically converts containers to alurity modules, adding the necessary logic for their interoperability with the overall infrastructure.

% Analyze/compare it to existing pentest distros such as backtrack ...

% Leveraging existing technologies for simulation and virtualization as opposed to reinventing the wheel ...

% Scalability beyond scenarios faced so far might require the use of multiple machines either physically or in the cloud. Orchestration mechanisms including Kubernetes might be explored for future efforts...

% Expose limitations of network connectivity abstractions across multiple platforms (Linux, Mac OS and Windows, mainly)....

% Hint that network simulation is at the moment reaching its bottom line and that emulation using VMs might be worth it.

% Connect with gym_gazebo ...


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONCLUSIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Conclusions}


% Future work, improve Windows support.

% Documentation is a missing item 

% The toolbox will automatically construct your security environment and preserve it across runs. 

% GUI/UI customer feedback. A first attempt to do so is available at alurity web page with selector...

%Altogether, this leads to the following research question: given the increasing complexity of robotic systems, how can we protect them from cyber-threats? Inspired by the popular adage \emph{"the best defense is a good offense"}, the present work attempts to answer this question by focusing on offensive practices yet, given the time-consuming requirements of traditional offensive security approaches \cite{ghanem2018reinforcement, niculaelearning2018, schwartz2019autonomous}, the answer might not be straightforward and require further automation.\\


In this study we presented \emph{alurity}, a modular and composable toolbox for robot cybersecurity that ensures that both roboticists and security researchers have a common, consistent and easily reproducible development environment. We described the architecture of \emph{alurity} including its capabilities for virtualization. We also described additional features that facilitate the security process and cooperation across teams, namely flows and pipelines. We then presented four real use cases conducted with \emph{alurity} and shared some lessons learned, emphasizing that simulation appears to speed up significantly cybersecurity research in robotics.

The lack of documentation for \emph{alurity} is currently the biggest hurdle  preventing us from disclosing it to a wider audience. Future work should focus on this. We also plan to look into preserving the state of the simulated scenarios across runs, as well as improved Windows support.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{ExploitFlow}
\showkeysfalse  % Disable keys    
\label{tools:exploitflow}
\showkeystrue  % Enable keys    

\subsection{Introduction}

Robots are often insecure and fully unprotected. The rationale behind this is fourfold: first, defensive security mechanisms for robots are still in their early stages, not covering the complete threat landscape. Second, the inherent complexity of robotic systems makes their protection costly, both technically and economically. Third, robot vendors are currently not taking responsibility in a timely manner, extending the zero-days exposure window (time until mitigation of a zero-day) to several years on average \cite{mayoral2019industrial}. Fourth, contrary to the common‐sense expectations and similar to Ford in the 1920s with cars, most robot manufacturers oppose or difficult robot hardware repairs and software patching. They employ planned obsolescence practices to discourage repairs and evade competition. In addition, it is observed how most manufacturers keep forwarding the cyber security problems to the end-users of these robotic machines, further obstructing the security landscape in robotics. Security is not a product, but a process that needs to be continuously assessed in a periodic manner, as systems evolve and new cyber-threats are discovered. Automation is crucial to tackle this problem. Specially, given the lack of security professionals and how long it takes to train qualified security researchers.

Against the current overwhelming insecurity landscape in robotics, this research paper advocates for offensive security methods for robots. These methods are necessary to understand attackers' behavior, to train defensive mechanisms and ultimately, to help protect existing systems by discovering flaws first. Building upon about a decade of robotics and empowering the use of Artificial Intelligence (AI) and Game Theory to automate attacks, this line of research aims to study how offensive AI-driven cyber security methods apply to robotics and allow to protect such systems in a feasible manner. In particular, this work presents \texttt{ExploitFlow} (\texttt{EF}), a modular library to produce cyber security exploitation routes (\emph{exploit flows}). \texttt{ExploitFlow} aims to combine and compose exploits from different sources and frameworks, capturing the state of the system being tested in a flow after every discrete action which allows learning attack trees that affect a given system.

\exploitflows's main motivation is to facilitate and empower Game Theory and Artificial Intelligence (AI) research in cyber security. A secondary motivation is to put \exploitflow in practice in an area wherein exploitation routes can help significantly secure complex systems via offensive cyber security mechanisms. Robotics is selected as the target area for this research, but other targets might be included in the future. To facilitate adoption, \exploitflows's syntax and architecture is inspired by TensorFlow\cite{abadi2016tensorflow}. 


%\newpage


% Define the colors for syntax highlighting
\definecolor{codegreen}{rgb}{0.3,0.6,0.3}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.5,0,0.33}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

% Define the style for the listings package
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},
    commentstyle=\color{codegreen},
    keywordstyle=\color{blue},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle,caption={\exploitflow usage example.}}
\begin{lstlisting}[language=Python]
import exploitflow as ef

flow = ef.Flow()      # Create a simple exploit flow
a = ef.placeholder()  # Instantiate a simple operation
print(flow.run(a))    # Run the flow and print results
\end{lstlisting}

\noindent A more complex exploitation route example is depicted below which performs reconnaissance locating multiple targets in the local area network and then conducts scans on each one of them to fill up the state:

\lstset{style=mystyle,caption={\exploitflow example doing multi-target reconnaissance. A exploit flow is built that performs reconnaissance locating multiple targets in the local area network and then conducts scans a targeted scan to \texttt{192.168.2.10} to fill up a state object that can then be used for reasoning.}}
\begin{lstlisting}[language=Python]
import exploitflow as ef

flow = ef.Flow()
init = ef.Init()
recon = ef.Targets()  # Build MSF reconnaissance exploit
versions = ef.Versions(ports=ef.state.TARGET_PORTS_COMPLETE)

# initialize state and pass it over a recon action
# resulting flow should deliver a state annotated
# with the results from the reconnaissance step
state = flow.run(init * recon * versions, target="192.168.2.10")
\end{lstlisting}

To simplify exploitation, \exploitflow represents each action in an exploitation route with the superclass Exploit, which includes reconnaissance and control actions\footnote{We are well aware that, strictly speaking, reconnaissance scripts don't meet the formal definition of an exploit. However, we still insist on grouping all actions under the same common class (Exploit) to simplify the production of exploitation flows (routes).}. Exploits are grouped into six major categories, inspired by the security kill chain\cite{lockheed2011}. \exploitflow is a modular, extensible library that accepts connectors for other exploitation frameworks and/or individual exploits, and is composable. \exploitflow is not an exploitation framework, but a tool to produce cybersecurity exploitation routes, which empowers research in Game Theory and Artificial Intelligence (AI) in cybersecurity.\\

\begin{figure}[b!]
    \centering % Centers the figure

    \begin{tikzpicture}[node distance=2cm, auto, scale=0.55, transform shape]
        % Styles for nodes and lines
        \tikzstyle{box} = [rectangle, draw, fill=gray!20, text centered, rounded corners, minimum height=2.5em, minimum width=3cm]
        \tikzstyle{emphasize} = [box, fill=blue!30, draw=blue, line width=1.5pt]
        \tikzstyle{line} = [draw, -{Latex[scale=1.2]}]
        \tikzstyle{deemphasize} = [opacity=0.3]
        \tikzstyle{innerComp} = [rectangle, draw, fill=orange!30, text centered, minimum height=1.5em, minimum width=3em]
    
        % Nodes
        \node[box] (U) {User};
        \node[emphasize] (EF) at (11cm,0) {1. ExploitFlow}; 
        \node[box, deemphasize, below left=4cm and 2.5cm of EF] (PentestGPT) {2. PentestGPT};
        \node[box, deemphasize, below=8cm of EF] (PentestPerf) {3. PentestPerf};
        \node[box, right=3cm of EF] (T) {Target};
    
        % Inner components of EF
        \node[innerComp, above=2.5cm of EF, xshift=-4cm] (exploit) {exploit};
        \node[innerComp, right of=exploit] (flow) {flow};
        \node[innerComp, right of=flow] (graph) {graph};
        \node[innerComp, right of=graph] (adapters) {adapters};
        \node[innerComp, right of=adapters] (models) {models};
        \node[innerComp, right of=models] (state) {state};
        
        % Dashed lines connecting EF to inner components
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (exploit);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (flow);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (graph);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (adapters);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (models);
        \draw[dashed, shorten <=5pt, shorten >=5pt] (EF) -- (state);
    
        % Lines
        \path[line] (U) -- node[font=\small, midway, sloped, above] {programatically in Python} (EF); 
        \path[line, deemphasize] (U) edge[bend right=40] node[font=\small, sloped, below, opacity=0.5] {goal description in text} (PentestGPT);
        \path[line, deemphasize] (PentestGPT) edge[bend right=20] node[font=\small, sloped, below] {exchange exploit tree} (EF);
        \path[line, deemphasize] (EF) edge[bend left=20] node {} (PentestGPT);
        \path[line, deemphasize] (EF) -- node[font=\small, sloped, above, opacity=0.5] {Benchmarks an exploit flow} (PentestPerf);
        \path[line] (EF) -- (T);
        \path[line] (T) -- (EF);
    
        % Group/box around EF and PentestGPT
        \node[rectangle, fill=gray!5, draw, dashed, deemphasize, fit=(EF) (PentestGPT), inner sep=1cm] (group) {};
        \node[anchor=north west, deemphasize, inner sep=0.5cm] at (group.south west) {4. Malism};
    
        % re-draw Nodes
        \node[box] (U) {User};
        \node[emphasize] (EF) at (11cm,0) {1. ExploitFlow}; 
        \node[box, deemphasize, below left=4cm and 2.5cm of EF] (PentestGPT) {2. PentestGPT};
        \node[box, deemphasize, below=8cm of EF] (PentestPerf) {3. PentestPerf};
        \node[box, right=3cm of EF] (T) {Target};
    
        % Legend
        \begin{scope}[node distance=0.3cm, font=\footnotesize]
            \coordinate (legendOrigin) at (-4,-6); % Set the position for the start of the legend
            \node[box, right=0.3cm of legendOrigin, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendBox) {}; 
            \node[right=0.3cm of legendBox] {External entity};
    
            \node[box, below=0.2cm of legendBox, fill=gray!5, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (otherpapers) {}; 
            \node[right=0.3cm of otherpapers] {Other chapters};
    
            \node[emphasize, below=0.2cm of otherpapers, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendEmphasize) {};
            \node[right=0.3cm of legendEmphasize] {This contribution};
    
            \node[innerComp, below=0.2cm of legendEmphasize, minimum height=1.5em, minimum width=1.5em, text width=1.5em] (legendInner) {};
            \node[right=0.3cm of legendInner] {Inner Component};
        \end{scope}
    \end{tikzpicture}
        
    \caption{Architecture of our framework to develop a fully automated penetration testing tools, \framework{}. 
        %Figure depicts the various interaction flows that an arbitrary \texttt{User} could follow using \framework{} to conduct penetration testing (pentest) a given \texttt{Target}. \textbf{1. (this paper)} Corresponds with \ef{}, a modular library to produce security exploitation routes (\emph{exploit flows}) that captures the state of the system being tested in a flow after every discrete action. \textbf{2.} Corresponds with \tool{}, a testing tool that leverages the power of LLMs to produce testing guidance (heuristics) for every given discrete state. \textbf{3.} \pentestperf is a comprehensive penetration testing benchmark to evaluate the performances of penetration testers and automated tools across a wide array of testing targets. \textbf{4.} captures \framework{}, our framework to develop fully automated penetration testing tools which we name \emph{cybersecurity cognitive engines}
    }
    \label{figure:cybersecurity_cognitive_engine:exploitflow} % Label to reference the figure elsewhere
\end{figure}

\noindent With this understanding, \exploitflow aims to contribute to unlocking the potential of modern machine learning approaches and developing a fully automated penetration testing framework that helps produce cybersecurity cognitive engines. Our overall architecture is depicted in Figure~\ref{figure:cybersecurity_cognitive_engine:exploitflow}, which shows our work thus far and our planned contributions for the near future. Figure depicts the various interaction flows that an arbitrary \texttt{User} could follow using \framework{} to conduct penetration testing (pentest) a given \texttt{Target}. \textbf{1.} (this contribution) Corresponds with \ef{}, a modular library to produce security exploitation routes (\emph{exploit flows}) that captures the state of the system being tested in a flow after every discrete action. \textbf{2.} Corresponds with \tool{}, a testing tool that leverages the power of LLMs to produce testing guidance (heuristics) for every given discrete state. \textbf{3.} \pentestperf is a comprehensive penetration testing benchmark to evaluate the performances of penetration testers and automated tools across a wide array of testing targets. \textbf{4.} captures \framework{}, our framework to develop fully automated penetration testing tools which we name \emph{cybersecurity cognitive engines}. Our proposed framework, \framework{}, is designed to enable a user without in-depth security domain knowledge to create their own cybersecurity cognitive engine that helps conduct penetration testing over an extensive range of targets. This framework comprises three primary components:
\begin{enumerate}

% ExploitFlow
\item \ef{} (\textbf{this contribution}): A modular library to produce cyber security exploitation routes (\emph{exploit flows}). \ef{} aims to combine and compose exploits from different sources and frameworks, capturing the state of the system being tested in a flow after every discrete action which allows learning attack trees that affect a given system. \ef{}'s main motivation is to facilitate and empower Game Theory and Artificial Intelligence (AI) research in cyber security. It provides a unique representation of the exploitation process that encodes every facet within it. Its representation can be effectively integrated with various penetration testing tools and scripts, such as Metasploit~\cite{moore2003metasploit} to perform end-to-end penetration testing. Such a representation can be further visualized to guide the human experts for the reproduction of the testing process. 

% PentestGPT
\item \tool{}: An automated penetration testing system that leverages the power of LLMs to produce testing guidance and intuition at every given discrete state. It functions as the core component of the \framework{} framework, guiding the LLMs to efficiently utilize their domain knowledge in real-world testing scenarios.

% PentestPerf
\item \pentestperf: A comprehensive penetration testing benchmark developed to evaluate the performance of penetration testers and automated tools across a wide array of testing targets. It offers a fair and robust platform for performance comparison.
\end{enumerate}

\noindent The harmonious integration of these three components forms an automated, self-evolving penetration testing framework capable of executing penetration tests over various targets, \framework{}. This framework to develop fully automated penetration testing tools, which we name \emph{cybersecurity cognitive engines}, aims to revolutionize the field of penetration testing by significantly reducing the need for domain expertise and enabling more comprehensive and reliable testing.\\


%provide a short summary of your methods and obtained results.
Contributions of this section are two-fold: first, we present for the first time the implementation and use of \exploitflow as a tool to build security exploitation routes. Second, we present the results obtained while creating an artificial agent powered by \exploitflow, that is able to locate exploits affecting the various robotic systems presented to the agent, while minimizing the amount of network traffic and attacks generated (exploits attempted). Q-Learning is used as the learning model and compared against two baselines: a) brute force and b) human expert. The source code including both the \exploitflow implementation as well as the machine learning experiments are available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow}.\\

Results presented below in section \ref{sec:evaluation} hint that \exploitflow is usable and useful for exploring ML use in the context of robot cybersecurity. Three actors are evaluated: the brute-force actor obtains a {\color{red!30!white}\texttt{-2680}} cumulative reward (see \ref{sec:learningmodel} for an explanation of the reward structure), the human expert {\color{blue!30!white}\textbf{\texttt{8}}} and the autonomous agent using value-based Reinforcement Learning (RL) {\color{green!30!white}\textbf{\texttt{100}}}. Attacks graphs shown hint that while the human expert iterates over reconnaissance exploits to introspect the networking scenario, the agent directly learns to submit the exploit that triggers a favourable reward and then iterates over an Idle action to maximize resulting reward (obtaining maximum possible, in fact). This overfitting behavior is a shortcoming to tackle in future work, since it impedes generalization across new testing environments. Overall, \exploitflow is demonstrated by creating an artificial agent powered by \exploitflow that is able to locate exploits affecting the target robotic systems presented to the agent, using value-based Reinforcement Learning (Q-Learning ) and while minimizing the amount of network traffic and attacks generated (exploits attempted). \exploitflow also demonstrates how the state of the system being tested is captured after every discrete action, which allows reasoning, keeping track of action/state pairs, and producing attacks trees affecting a given system. Ultimately, we present in Figure \ref{figure:cybersecurity_cognitive_engine:exploitflow} the architecture of our framework to develop a fully automated penetration testing tools, \framework{}, which we name cybersecurity cognitive engines, and which uses \exploitflow at its core.

%\section{Learning task}
%\label{sec:learningtask}
%
%\subsection{The task to learn}
% what are you going to do?
%The \emph{task to learn} consists of creating an artificial agent powered by \exploitflow that is able to locate exploits affecting the various robotic systems presented to the agent, while minimizing the amount of network traffic and attacks generated (exploits attempted).
%
%\subsection{Training experience}
% where is your training experience coming from? why do you think that your data can actually be used to solve the problem? Provide examples of your data and use them to explain your learning task.
%
%Target robotic systems will be simulated via Operating System (OS)-virtualization. In particular, building upon prior work\cite{mayoral2020alurity} Docker will be used to containerize the file systems of target robots. Targets will be realistic and will capture robotic systems currently being used in production. Training experience will be collected experimentally via Reinforcement Learning (RL) and by having the artificial agent interact with each one of the corresponding targets. 
%
%Future work and extensions will consider selecting additional targets (e.g. vulnerable web servers and/or connected machines exposing vulnerable services) in the form of Capture-The-Flag (CTF) environments, which as demonstrated in past work \cite{mendia2018robotics}: 1) aligns well with the OS-virtualization approach selected, 2) will allow the agent to generalize its behavior towards more cyber security environments and 3) will help further demonstrate the use of \exploitflow for Game Theory and AI security research in robotics.

%\subsection{Performance measure}
% how are you going to measure your success? which measures will be used and why? how can results returned by your measures be interpreted in the context of your problem, e.g. precision=0.7 is it good or bad?

%Performance of the artificial agents will be benchmarked against two baselines: a) brute force and b) a human cyber security experienced performer. Benchmark will consist of various indicators with at least:

%\begin{itemize}
%    \item \textbf{1. Attack tree}: An attack tree is a hierarchical diagram that represents the potential paths an attacker can take to compromise a system or achieve a specific goal. In cyber security, an attack tree is used as a tool to analyze and understand the security of a system, identify potential vulnerabilities, and develop mitigation strategies. \exploitflow allows to easily produce the attack tree given an exploitation flow and to compare it against other trees. Aspects to consider in the tree include depth and number of leaves (number of vulnerabilities found).
%    \item \textbf{2. Cumulative reward}: The cumulative reward of each agent (and each one of the baselines) will be considered as an indicator. Note each action that generates network traffic will correspond with a negative reward (this includes reconnaissance attempts, exploitation attempts, privilege escalation, lateral movement, etc.). Negative rewards will be proportional to the (security) severity of the network interaction. For example, reconnaissance attempts will generally have a low negative rewards, whereas exploitation attempts will have a significantly higher negative rewards. Rationale behind this is to provide additional realism to the analysis, as most modern Intrusion Detection Systems (IDS) will flag exploitation attempts rapidly. If an exploitation attempt results in discovering successfully a vulnerability, then that action will result in a positive reward.
%\end{itemize}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Methodology}


% describe the data you are using in the project and provide examples. what kind of data you are using, where does it come from? what are the properties of your data, like balance, missing values, scale, etc., and what are you going to do about it? what kind of preprocessing, filtering, augmentation, or other manipulations are you applying in the project?  

This section describes the research approach, including the data used for the learning task and the learning model. Subsection~\ref{cornerstones} will first set the context, the current state of the art and will highlight the lack of available datasets for robot cybersecurity study. Section~\ref{datagen} will then discuss our approach for data generation through CTF-like OS-virtualized environments to generate realistic robotics networking data and what kind of preprocessing and other manpulations were applied to it for the learning task. Finally, Section~\ref{sec:learningmodel} will present an overview of our learning approach and the model used.

%\newpage

\subsubsection{Biographical cornerstones in machine learning applied methods to robot cybersecurity}

\showkeysfalse  % Disable keys    
\label{cornerstones}
\showkeystrue  % Enable keys


%The following presents a summary of some of the most relevant and recent research articles related to offensive cybersecurity approaches that leverage machine learning:

%\begin{hypothesis}
%\label{hyp:offensive_approach}
%Complexity difficulties security. The inherent complexity of robotic systems, which leads to wide attack surfaces and a variety of potential attack vectors will be tackled with a reverse defensive approach, an offensive one.
%\end{hypothesis}

%\begin{hypothesis}
%\label{hyp:mlandgt}
%Scalability problems in offensive security will be addressed by focusing on the development of an autonomous, end-to-end offensive security assessment algorithm that leverages Machine Learning and Game Theory.
%\end{hypothesis}


%\noindent This thesis will dive into robot cyber security and study how traditional and modern offensive methods apply to robotics, delivering a new angle to protect such systems. Scalability is one of the core problems of offensive security assessments (red teaming, penetration testing, etc.) as of now \cite{applebaum2016intelligent, applebaum2017analysis}. To this question, the research herein proposed will review and create new mechanisms and techniques that leverage Machine Learning and Game Theory allowing for the full automation of offensive security assessments. This research will also argue and challenge the underlying ethics of the security community when applied to robotics. Particularly, \emph{de facto} standards and conventions on security outcomes and disclosures will be assessed and challenged, with a critical non-vendor-centered attitude. Ultimately, given the novelty of the topic itself, a relevant number of contributions are expected in the form of blueprints that will empower future research.

%The following sections describe this thesis proposal in detail. Section \ref{sec:sota} discusses the literature review and foundations of the research. Section \ref{sec:objectives} elaborates on the research objectives and the approach followed. Finally, section \ref{sec:workplan} presents prior research actions by the author, results during the first year of the PhD and expected future publications.

%In an attempt to raise awareness and create some base formal studies and tools, this research proposal's objective is to study how offensive cyber security methods apply to robotics. In particular, this proposal aims to study how traditional methods in offensive security are applied to robotics. Such methods include penetration testing, red teaming, automated attack planning or advanced persistent threats amongst others. In addition, this study will cover ethics and defensive security mechanisms that protect systems, networks and operations. Such is necessary for implementing offensive methods and understanding the underlying legal boundaries. Ultimately, this study will look into how to automate and optimize offensive cyber security attacks targeting robots,  making use of Artificial Intelligence and Game Theoretic approaches.\\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% State of the Art 
% 
% The State of the Art, also known as the Literature Review (or Foundations), serves a cluster of very important aims. First of all, it demonstrates that you have built a solid knowledge of the field where the research is taking place, that you are familiar with the main  issues  at  stake,  and  that  you  have  critically identified  and  evaluated  the  key literature. On the other hand, it shows that you have created an innovative and coherent view integrating and synthesising the main aspects of the field, so that you can now put into perspective the new direction that you propose to explore. The State of the Art must give credit to the authors who laid the groundwork for your research, so that when, in the following chapter, your research objectives are further clarified, the reader is able to recognise beyond doubt that what you are attempting to do has not been done in the past and that your research will likely make a significant contribution to the literature. The State of the Art is usually the more extensive part of a research proposal, so it will expectedly  develop  over  various  paragraphs  and  sub-paragraphs.  It  should  be accompanied by comprehensive references, which you list at the end of the proposal. Ideally,  all  influential  books,  book  chapters,  papers  and  other  texts  produced  in  the 


%\vspace{-4cm}

\begin{comment}
    

\startchronology[startyear=2005,stopyear=2025,height=1.0ex]

\chronoevent[textwidth=7cm,markdepth=140pt]{08/2022}{\small Hierarchical reinforcement learning for efficient and effective automated penetration testing of large networks \cite{ghanem2022hierarchical}}

%\chronoevent[textwidth=8cm,markdepth=-150pt]{2020}{\small \bf Modeling penetration testing with reinforcement learning using capture-the-flag challenges: trade-offs between model-free learning and a priori knowledge \cite{zennaro2020modeling}}

\chronoevent[textwidth=3cm,markdepth=10pt]{2005}{\small MulVAL: A Logic-based Network Security Analyzer \cite{ou2005mulval}}

\chronoevent[textwidth=5cm,markdepth=-20pt]{2013}{\small PEGASUS: A policy search method for large MDPs and POMDPs \cite{ng2013pegasus}}

\chronoevent[textwidth=3cm,markdepth=25pt]{2016}{\small Intelligent, automated red team emulation \cite{applebaum2016intelligent}}

\chronoevent[textwidth=4cm,markdepth=85pt]{09/2019}{\small NIG-AP: a new method for automated penetration testing \cite{zhou2019nig}}

\chronoevent[textwidth=6cm,markdepth=-95pt]{12/2019}{\small Reinforcement learning for efficient network penetration testing \cite{ghanem2020reinforcement}}

\chronoevent[textwidth=4cm,markdepth=-30pt]{2020}{\small \bf Automated penetration testing using deep reinforcement learning \cite{hu2020automated}}

\chronoevent[textwidth=3cm,markdepth=20pt]{2021}{\small Automating post-exploitation with deep reinforcement learning \cite{maeda2021automating}}

%\chronoevent[textwidth=8cm,markdepth=200pt]{2023}{\small GAIL-PT: An intelligent penetration testing framework with generative adversarial imitation learning \cite{chen2023gail}}

\stopchronology
\end{comment}

System complexity is the enemy of security. It is very difficult to assure no vulnerabilities in a system that an attacker could exploit. In robotics, the reality is even more concerning, as robots are complex systems, with wide attack surfaces and wherein there is no culture of security yet. As studied in previous work~\cite{kirschgens2018robot, mayoralrvd}, except few vendors and selected actions, no real concern has been shown for security in robotics. Offensive security methods (such as pentesting or red teaming) play an important part in the security lifecycle. In these engagements, as introduced by Applebaum~\cite{applebaum2017analysis}, security teams try to break into an organization’s assets, identifying vulnerabilities along the way. Red teams take this concept even further, trying to fully emulate what real adversaries do: instead of just compromising the network and identifying vulnerabilities, they have a larger goal that requires significant post-compromise work.


Various authors, including those summarized above took note of this, and started leveraging offensive mechanisms to tackle the cybersecurity problem. In particular, \cite{ghanem2018reinforcement, niculaelearning2018, schwartz2019autonomous} among others started using machine learning to automate the penetration testing task, presenting different levels of automation. Most of the authors use rather simple  neural network architectures, many leveraging Deep Q-Learning (DQN) and mostly involving few hidden layers, besides the input and output ones. This hints about the fact that the tasks learned are rather simple, and a simplification of the complete penetration testing activities. Something coherent across most of these studies is the lack of consistency concerning the representation of the state space for cybersecurity research purposes in ML. Connected to it, we found that most cited authors above use inconsistent datasets.  Though various popular \emph{security-oriented networking datasets} exist (see \faGithub~  \url{https://github.com/shramos/Awesome-Cybersecurity-Datasets}) most of the authors reviewed seem to discard these and instead choose to generate their own data via either abstractions (simplified models) or simulated/emulated environments. Further research hinted that rationale behind this is two-fold:

\begin{enumerate}
    \item {Capturing networking data in a scalable manner is non-trivial (and an open problem)}
    \item {Cybersecurity environments are highly non-structured and interactive}
\end{enumerate}


In this work, we fail to locate a dataset that could serve the research goals. Deploying offensive cybersecurity approaches in the complex robotics field presents quite a challenge, given its novelty. Also, because the robotics realm is prohibitive: cost, repeatability, and expertise all make it difficult to consistently produce offensive security datasets. Following from this, and similar to some of the cited work above. To proceed with this research, we attempted addressing the two identified hurdles cited above by collecting synthetic data directly from a realistic OS-virtualized scenario with multiple robotic targets. The following sections discuss our approach.



\subsubsection{Synthetic data generation through CTF-like OS-virtualized environments}

\paragraph{Data generation}
\showkeysfalse  % Disable keys    
\label{datagen}
\showkeystrue  % Enable keys


Obtaining a proper dataset is crucial and specially hard in certain areas, such as the unstructured robotics or cybersecurity. The intersection of both presents an even more difficult challenge. In particular for security, automating offensive cyber security practices constitutes a non‐trivial problem because of the range and complexity of actions that a human expert may attempt, which hampers putting together representative datasets. The authors of \cite{zennaro2020modeling} acknowledge this and focus their attention on simplified penetration testing problems expressed in the form of Capture The Flag (CTF) hacking challenges. They tackle the \emph{dataset production} problem by leveraging existing CTF environments, which they modify to adapt to modern RL \emph{gyms} which produce a reward after an agent performs an action. This way, authors are able to \emph{produce} relevant input data (which serves as datasets) for the learning offensive cyber security practices in selected target scenarios. The research herein will reproduce the approach followed at \cite{zennaro2020modeling} with relevant  extensions meant for modeling robots. The reader should note that while pure networking (for security purposes) modeling can easily be done with virtualization (e.g. OS-virtualization such as Docker, or VMs which are commonly used), robotic environments require a significantly more complex abstraction set, which elevates the complexity of building such CTF environments. To address this problem, the present work builds on top of some of \cite{mayoral2020alurity}, which provides a toolbox for robot cybersecurity concerning. Altogether, we are able to build OS-virtualized CTF environments with the target robots that allow performing RL on them. 

Data is thereby generated as synthetic and directly from the simulated robotic environments, each of which can fit a different challenge, or CTF game. The data corresponds to the simulated networking interactions between peers. The following describes how such networking dataflow is abstracted away for learning purposes.

% describe in here how data's captured for processing
\paragraph{Data pre-processing}

Learning from computer networking data requires relevant data pre-processing, as the amount of information is overwhelming. The following presents our initial assumptions while considering networking data pre-processing. 

Let's assume the following:
\begin{itemize}
    \item At each time-step, the network is captured by a \texttt{State} class. On its simplest form, each \texttt{State} is represented by a dictionary, each key corresponding with an IP address and holding a sub-state class which captures (for each IP) a) exploits launched against the network and b) port status (open/closed, versions, cpe, etc.).
    \item One-hot encoding is used as the safest approach to interface with the learning model. Others considered included label encoding and binary encoding. While the latter produced shorter representations, binary encoding might not be suitable for all machine learning algorithms. In binary encoding, although categories are converted into numbers, there is an arbitrary ordering introduced in the categories, which might mislead some algorithms into thinking that there is a relationship between different categories. One-hot encoding instead  doesn't have this issue as it uses binary vectors to represent categories, at the cost of increasing the dimensionality of the dataset.        
\end{itemize}

Given these assumptions, we considered initially the following:

\begin{itemize}
    \item $y = 255$, number of IPs considered (a complete minor subnet)
    \item $n = 424$, number of ports monitored, each represented by $l = 1$ bit to capture its state (open/close)
    \item $m = 12$, number of exploits considered, each represented by $b = 1$ bits (launched/not-launched), discarding capturing the success/failure of each exploit to model better the uncertainty often encountered in cybersecurity.
    \item $s = 0$ bits capturing the system information for each IP (OS version, and other meta-data obtained while doing reconnaissance)
\end{itemize}

These assumptions, which already introduce a significant simplification, while one-hot encoded already lead to the following number of elements while encoding the \texttt{State}:

\begin{equation*}
    \begin{split}
y \cdot [n \cdot (n + l) + \cdot (m + b) + s] = \\
255 \cdot [424 \cdot (424 + 1) + 12 \cdot (12 + 1) + 0] = \\
256 \cdot 180,356 = 46,171,136
    \end{split}
\end{equation*}

This leads to a setup which is non-feasible computationally. These initial assumptions had to change. We had to significantly increase abstractions (and reduce complexity in terms of network-scope) to make computations tractable in modern general-purpose computers. In particular we used $y = 7$, $n = 9$, $l = 1$, $m = 12$, $b = 1$ and $s = 0$ leading to:

\begin{equation*}
    \begin{split}
y \cdot [n \cdot (n + l) + \cdot (m + b) + s] = \\
7 \cdot [9 \cdot (9 + 1) + 12 \cdot (12 + 1) + 0] = \\
7 \cdot 246 = 1,722
    \end{split}
\end{equation*}


Preserving the modularity principles of \exploitflows, all the above is implemented by a \texttt{State} class that can easily be extended, overwritten and/or modified per each experiment independently. The listing \ref{lst:state} shows an example implementing a variant of \texttt{State} called \texttt{State\_v2}:



% Describe how Exploitflow hosts metadata on each exploit


\subsubsection{Learning model}  % aka, the theoretical part
\showkeysfalse  % Disable keys    
\label{sec:learningmodel}
\showkeystrue  % Enable keys

As described above, most of the prior art reviewed use rather simple neural network architectures for cybersecurity automation and machine learning, many leveraging Deep Q-Learning (DQN) and mostly involving few hidden layers, besides the input and output ones. In a way, this could be understood as an indicator that the field is still mostly immature (from an ML-perspective) and that simple problems are being explored, which don't demand complex models. In light of this and particularly following the trend established by \cite{zennaro2020modeling} which focus on scalability, rather than complexity of the problem to solve using a more \emph{explainable} model, we adopt a similar approach and leverage reinforcement learning with simple table-based Q-Learning as a model.\\
\newline
Besides Q-Learning, the following hyperparameters are used consistently across our machine learning efforts: learning rate (alpha, $\alpha$) = 0.1, discount factor (gamma, $\gamma$) = 0.9, exploration factor (epsilon, $\epsilon$) = 0.1.\\
\newline
Finally, the following reward scheme was applied:
\begin{itemize}
    \item Non-exploits, like idle (no action) and related were assigned a reward of $0$, helping the agent to learn that idle might be appropriate given certain networking conditions.
    \item reconnaissance (both fingerprinting and footprinting) actions were assigned a reward of $-10$ by default, and an extra $-1$ for each IP target impacted while incurring in footprinting. This way, we penalize the additional networking traffic generated, which can help Intrussion Detection Systems (IDS) detect malicious activity.
    \item Formal offensive exploits were assigned a reward of $100$ when successful, and $-100$ if failed.    
\end{itemize}

% literature overview: which models from the literature are suitable for this problem given your data and why? which algorithms can be used to train them? how these models are related to your hypothesis? 
%
%present an overview of your approach: what steps are executed in the learning pipeline? which hyperparameters of the learning algorithm are available and how they can influence the results? 
%
% You must show that you applied methods considered during the semester to the selected problem. Feel free to include any figures or tables helping to describe your method and compare it with others. If you use information from other sources, please cite it properly.



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Implementation}
%\label{sec:implementation}

% how did you implement your approach? which tools were used? show interesting snippets or present your algorithms

%Implementation was performed in Python, as an extension of \exploitflow (which is coded in Python as well) and in a separate file with standardized interfaces for use. Models abstracted using these interfaces can easily be swapped and tested. Our table-based Q-Learning model presents the form depicted in listing \ref{lst:qlearning}. An extension of this implementation to use other models that leverage artificial neural networks (e.g. DQN) is judged trivial if/when leveraging popular machine learning frameworks such as \emph{TensorFlow}. An archive of past such implementations and examples developed by the author of this report is available at \faGithub~  \url{https://github.com/vmayoral/basic_reinforcement_learning}.


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Evaluation}

\showkeysfalse  % Disable keys    
\label{sec:evaluation}
\showkeystrue  % Enable keys    


Evaluation was performed in a simulated scenario involving the following robotic systems presented in Figure \ref{figure:exploitflow_test_scenario}. Target objective of the learning effort is to compromise the Universal Robots UR3 collaborative manipulator using \href{https://github.com/aliasrobotics/RVD/labels/robot%20component:%20Universal%20Robots%20Controller?page=4&q=is%3Aopen+label%3A%22robot+component%3A+Universal+Robots+Controller%22}{well known security vulnerabilities} affecting this robotic system. In particular, an exploit for compromising the robot using the \href{https://github.com/aliasrobotics/RVD/issues/672}{RVD\#672} (hard-coded public credentials for controller) vulnerability will be used. Three situations were considered and described below:

\begin{figure}[h!]
    \includegraphics[width=0.8\textwidth]{figures/scenario_simplified.png}
    \centering
    \caption{CTF-like OS-virtualized robotic environments involving 4 robotic targets: a robotic brain powered by ROS 2, another powered by ROS, a UR3 cobot manipulator and a PX4 drone.   %Source code to reproduce this environment is available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow/blob/main/.devcontainer/docker-compose.yml}
    }
    \label{figure:exploitflow_test_scenario}
\end{figure}



% present and visualize results of your evaluation, explain what do your results mean, why was your approach successful, why not? compare it to some baseline either implemented yourself or from the literature, blogs, Kaggle, etc.

\subsubsection{Human-expert penetration tester}

A human-expert was considered by using \exploitflow programatically, and manually programming an exploitation route for the best-case scenario. Exploitation route is achieved using the code snippet at listing \ref{lst:human} (complete experiment available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow/blob/main/examples/9_exploitation_ur_human_expert.py}).

The execution of this exploitation flow leads to the attack graph depicted in Figure \ref{fig:humanexpert} and led to a cumulative reward of $8$.

\begin{figure}[h!]
    \includegraphics[width=0.8\textwidth]{figures/1_human_expert.png}
    \centering
    \caption{Depiction of the attack graph produced by a human expert while executing the manually-written best-case exploit flow.}
    \label{fig:humanexpert}
\end{figure}


\subsubsection{Autonomous agent powered by Q-Learning}

An artificial agent powered by \exploitflow is able to locate exploits affecting the target robotic system, while minimizing the amount of network traffic and attacks generated (exploits attempted) using its table-based Q-Learning model. Exploitation route is learned using the code snippet at listing \ref{lst:agent} (complete experiment available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow/blob/main/examples/11_exploitation_ur_qlearning_instances.py}).


The execution of this exploitation flow leads to the attack graph depicted in Figure \ref{figure:ai_agent} and led to a cumulative reward of $100$.

\begin{figure}[h!]
    \includegraphics[width=0.8\textwidth]{figures/0_ai_agent.png}
    \centering
    \caption{Depiction of the attack graph produced by an autonomous agent powered by Q-Learning algorithm while executing the exploit flow that is derived from its learned value-function (table).}
    \label{figure:ai_agent}
\end{figure}

Implementation was performed in Python, as an extension of \exploitflow (which is coded in Python as well) and in a separate file with standardized interfaces for use. Models abstracted using these interfaces can easily be swapped and tested. Our table-based Q-Learning model presents the form depicted in listing \ref{lst:qlearning}. An extension of this implementation to use other models that leverage artificial neural networks (e.g. DQN) is judged trivial if/when leveraging popular machine learning frameworks such as \emph{TensorFlow}.

\subsubsection{Brute-force}

A brute force baseline (which often the case relates to what many novel pentesters do) is generated by launching all permutations of the selected available exploits against the scenario\footnote{In fact, a reduced "relevant" set was selected to make it computationally more tractable}. Exploitation route is created using the code snippet available at listing \ref{lst:brute} (complete experiment available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow/blob/main/examples/13_exploitation_ur_bruteforce.py}). The execution of this exploitation flow leads to a big attack graph (not shown here) and led to a cumulative reward of $-2680$.



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Conclusions}

In this section, we made notable contributions to the realm of robot cybersecurity by producing \exploitflow, a modular library to produce cyber security exploitation routes (\emph{exploit flows}) that allows combining and compose exploits from different sources and frameworks, and captures the state of the system being tested in a flow after every discrete action. This allows for further automated reasoning (by means of ML and Game Theory), as well as learning attack trees that affect a given system. Firstly, we introduced the novel implementation of \exploitflow, an innovative tool devised for crafting security exploitation routes. Furthermore, we successfully demonstrated \exploitflow by developing an artificial agent with it, that capably identifies exploits in various robotic systems, significantly minimizing both network traffic and the number of exploits attempted.

Using Q-Learning, we compared the efficiency of our model against two baselines: brute force and human expert. Interested readers can delve into the source code and machine learning experiments available at \faGithub~  \url{https://github.com/vmayoral/ExploitFlow}. \exploitflow's ability to capture the system state post every discrete action is paramount. It aids in logical reasoning, tracing action/state combinations, and generating attack trees for a specific system. To encapsulate our endeavors, Figure \ref{figure:cybersecurity_cognitive_engine:exploitflow} outlines the architecture of \framework{}, our automated penetration testing tool—termed as a cybersecurity cognitive engine—with \exploitflow as its foundational element.


\begin{figure}[h!]
\centering
\resizebox{0.8\textwidth}{!}{ 
\begin{tikzpicture}
\begin{axis}[
    xbar,
    xlabel={Cumulative reward},
    xlabel style={align=center},
    xmajorgrids=true, % Enable a grid
    grid style=dashed,
    ytick={1,2,3},
    yticklabels={Human expert, Autonomous agent (Q-Learning), Brute-force},
    nodes near coords,
    nodes near coords align={horizontal},
    nodes near coords style={font=\footnotesize},
    y tick label style={align=center, font=\small},
    cycle list={
        {fill=blue!30!white,draw=blue!30!black, line width=0.8pt}, % Human color
        {fill=green!30!white,draw=green!30!black, line width=0.8pt}, % RL color
        {fill=red!30!white,draw=red!30!black, line width=0.8pt}, % Brute-force color
    },
    height=10cm,
    bar width=0.7cm,
    enlarge y limits={abs=1},
    axis x line*=bottom, % Remove the box around the plot
    axis y line*=left,
    extra x ticks={-2500,-2000,-1500,-1000,-500,0},  % <-- add the ticks you need
    extra x tick style={tick label style={color=red}},
]
\addplot coordinates {(8,1)};
\addplot coordinates {(100,2)};
\addplot coordinates {(-2680,3)};

% Dashed lines extending to the top horizontal side with values
\addplot[dashed,sharp plot, line width=0.7pt] coordinates {(8,1) (8,5)} node [right] {};
\addplot[dashed,sharp plot, line width=0.7pt] coordinates {(100,2) (100,4)} node [right] {};
\addplot[dashed,sharp plot, line width=0.7pt] coordinates {(-2680,3) (-2680,5)} node [right] {};
\end{axis}
\end{tikzpicture}}
\caption{Cumulative reward obtained by three different actors (brute-force, Q-Learning, human expert) while attempting to compromise the target objective in the robot cybersecurity scenario of figure \ref{figure:exploitflow_test_scenario}}
\label{figure:cumulative_reward}
\end{figure}

% how can you evaluate the results of your work? what would you recommend for future steps?

\noindent Results of the three actors evaluated during this research are summarized in Figure \ref{figure:cumulative_reward}, depicting the cumulative reward of the exploit flow generated for each actor, respectively (see \ref{sec:learningmodel} for an explanation of the reward structure). The brute-force actor obtains a {\color{red!30!white}\texttt{-2680}} cum. reward, the human expert {\color{blue!30!white}\textbf{\texttt{8}}} and the autonomous agent using value-based Reinforcement Learning (RL) {\color{green!30!white}\textbf{\texttt{100}}}. While analyzing figures \ref{fig:humanexpert} and \ref{figure:ai_agent} it becomes apparent that while the human expert iterates over reconnaissance exploits to introspect the networking scenario, the agent directly learns to submit the exploit that triggers a favourable reward and then iterates over an Idle action to maximize the resulting reward (obtaining maximum possible, in fact). In light of results, we can conclude that the initial research objectives have been fulfilled. \exploitflow implementation was shown functional and demonstrated by creating an artificial agent powered by \exploitflow that is able to locate exploits affecting the target robotic systems presented to the agent, using value-based Reinforcement Learning (Q-Learning ) and while minimizing the amount of network traffic and attacks generated (exploits attempted).\\
\newline
Though results meet the initial goals, we must be critical towards identified shortcomings. The following hint a few directions werein future work could be allocated for further improvements:
\begin{itemize}
    \item First, current learned functions (value-based) overfit to the particular landscape of exploits available and would perform poorly the moment the networking configuration changes (e.g. IP addresses change). To overcome this,  training should be performed without the use of heuristics or simplifications and using \emph{changing} networking setups. Though this can be automated (e.g. creating varios CTF-like scenarios), it was beyond the scope of the current effort. A side-effect of this would be the explosion of the state-space, which would probably require to leverage other function representation models, such as artificial neural networks (as opposed to the current table).
    \item Second, as part of this \emph{overfitting} behavior mentioned, we acknowledge that it is unrealistic for the current autonomous agent to perform properly in the wild, as offensive cybersecurity always requires some level of (continued) reconnaissance. The current agent has not learned to do so. Reward shaping and various scenarios could help addressing this limitation.
    \item Third, the current one-hot encoding is not scalable (computationally very expensive) and alternatives must be explored if the networking \texttt{State} is to be better captured.
    \item Fourth, a better representation of the networking state at each timestamp is required to further scale learning. Ideas in this direction include incorporating machine-related metadata (OS, library versions extracted from finger- and foot-printing).
    \item Fifth and much relevance, there is a huge scalability problem (very costly engineering-wise) while generating datasets that helps autonomous agents learn which action to take next. Creating usable (by ML agents) exploits and scenarios takes a lot of expertise and time. Building appropriate scenarios requires qualified roboticists that understand the dynamics of robotic systems. Adapting exploits for use (or worse, creating new ones) requires cybersecurity experts to craft the right interfaces for automated learning use. To overcome this limitation, modern and popular Large Language Models (LLMs) can be utilized to produce both scenarios as well as exploits in the form/format required, significantly simplifying the effort to produce usable datasets and actions. Listing \ref{lst:llm} shows a hint about how LLMs could be leveraged to tackle this shortcoming. We refer interested readers to submodule 2. \tool{} of Figure \ref{figure:cybersecurity_cognitive_engine:exploitflow} for more details on this line of work.
    \item Sixth, and somewhat connected to the previous one, the heterogeneity of the security networking environments seems to require heuristics to interpret the networking \texttt{State} and take initial actions while tackling new security challenges in unseen environments. This is somewhat connected to the fact that it is unrealistic to capture all know-how concerning offensive attempts, as most is non-disclosed or in a format that can easily be digested and converted into datasets.  LLMs could also help on this regard, which is a topic worth researching.     
\end{itemize}

Ongoing efforts to tackle these shortcomings are being developed by the authors. Some available in-the-open and publicly (e.g. at \faGithub~ \url{https://github.com/GreyDGL/PentestGPT}), which will be treated in a later chapter. We also refer interested readers to Figure~\ref{figure:cybersecurity_cognitive_engine:exploitflow} to get a hint of the overall architecture of \framework{}, our framework to produce cybersecurity cognitive engines.
    


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/IV.attacking/X.case_studies.tex <==
\chapter{Case studies cyber-attacking robots}
\label{chapter:case_studies}


% Use case studies from website of Alias
% https://aliasrobotics.com/case-studies-robot-cybersecurity.php

\section{Introduction}

%This chapter will look at some of the robot cybersecurity case studies conducted throughout this research.

==> sections/V.automation/X.cognitive_engine.tex <==
\chapter{Automating offensive robot cybersecurity}
%, 
%
%building a cybersecurity cognitive engine
\label{chapter:cognitive_engine}

\kant[15-19] % Dummy text

% Malism, or push everything to the conclusion

